Control Barriers in Bayesian Learning of System Dynamics

This paper focuses on learning a model of system dynamics online while satisfying safety constraints. Our objective is to avoid offline system identification or hand-specified models and allow a system to safely and autonomously estimate and adapt its own model during operation. Given streaming observations of the system state, we use Bayesian learning to obtain a distribution over the system dynamics. Specifically, we propose a new matrix variate Gaussian process (MVGP) regression approach with an efficient covariance factorization to learn the drift and input gain terms of a nonlinear control-affine system. The MVGP distribution is then used to optimize the system behavior and ensure safety with high probability, by specifying control Lyapunov function (CLF) and control barrier function (CBF) chance constraints. We show that a safe control policy can be synthesized for systems with arbitrary relative degree and probabilistic CLF-CBF constraints by solving a second order cone program (SOCP). Finally, we extend our design to a self-triggering formulation, adaptively determining the time at which a new control input needs to be applied in order to guarantee safety.

==> old/SafeControl.tex <==

%Thm.~\ref{thm:CBC2-quanti34} in the appendix provides the expressions for mean and variance of $\mbox{CBC}_k^{(2)}$.

% \subsection{old stuff}
% Define the condition required for $h(\bfx)$ to be an Exponential CBF as,
% %
% \begin{align}
% \CBCtwo(\bfx; \bfu) &= \Lie_f^2h(\bfx) + \Lie_g\Lie_fh(\bfx)\bfu + K_\alpha [h(\bfx), \Lie_fh(\bfx)]^\top.
% \end{align}%
% % 
% 
% 
% In Section~\ref{proof:mean-var-of-cbc}, we show how to compute the distribution
% of Gaussian process $\bfz(\bfx; \bfu)$ and the mean and variance of $\LieTwo$ is
% given by
% %
% \begin{align}
%   \E[\LieTwo(\bfx;\bfu)]
%   &= 
%   \E[\grad \LieOne h(\bfx)]\E[\tdbff(\bfx; \bfu)]
%   + \tr(\grad[\cov( \LieOne h(\bfx)], \tdbff(\bfx; \bfu)))
%   \\
%   \Var[\LieTwo h(\bfx;\bfu)]
%   &= 
%   2\tr(\grad \cov(\LieOne h(\bfx), \tdbff(\bfx; \bfu)))^2
%     \nonumber\\
%   &+ 2 \grad \E[\LieOne h(\bfx)] \grad \cov(\LieOne h(\bfx), \tdbff(\bfx; \bfu)) \E[\tdbff(\bfx; \bfu)]
%     \nonumber\\
%   &+ \grad \E[\LieOne h(\bfx)] \Var[\tdbff(\bfx; \bfu)] \grad \E[\LieOne h(\bfx)]
%   + \E[\tdbff(\bfx; \bfu)]  H_xx \Var[\LieOne h(\bfx)] \E[\tdbff(\bfx; \bfu)]
%   \\
%   \cov(\tdbff(\bfx; \bfu), \LieTwo &h(\bfx;\bfu))
%   =
%     \grad \cov(\tdbff(\bfx; \bfu), \LieOne h(\bfx)) \E[\tdbff(\bfx; \bfu)]
%     + \Var(\tdbff(\bfx; \bfu)) \grad \E[\LieOne h(\bfx)]
%   \\
%   \cov(\LieOne(\bfx), \LieTwo &h(\bfx;\bfu))
%   =
%     \grad \cov(\LieOne(\bfx), \LieOne h(\bfx)) \E[\tdbff(\bfx; \bfu)]
%     + \cov(\LieOne(\bfx), \tdbff(\bfx; \bfu)) \grad \E[\LieOne h(\bfx)]
% \end{align}%
% % 
% 
% 
% The mean and variance of $\CBCtwo$ can be then computed as,
% %
% \begin{equation}\begin{split}%
% \mCBCtwo
% &= 
% \E[\LieTwo h(\bfx)]
%   + K_{\alpha}\begin{bmatrix} h(\bfx)
%    & \E[\LieOne h(\bfx)]
%    \end{bmatrix}^\top
% \\
% \VCBCtwo
% &=
% \Var[\LieTwo h(\bfx)]
% + K_{\alpha,2}\Var[\LieOne h(\bfx)]
% + 2 K_{\alpha,2} \cov(\LieOne h(\bfx), \LieTwo h(\bfx))
% \label{eq:mean-var-cbc}
% \end{split}\end{equation}%
% %
% 
% 
% We use one-sided Chebyshev inequality to bound the tail of the distribution with
% probability mass $1-\delta $.
% 
% For any random variable $X$ with finite variance $\sigma^2$, mean $\mu$, and
% for any scalar $\lambda > 0$,
% %
% \begin{align}
%     \Prob(X - \mu \ge \lambda )
%     &\le \frac{\sigma^2 }{\sigma^2 + \lambda^2}
%     &
%     \Prob(X - \mu \le - \lambda )
%     &\le \frac{\sigma^2 }{\sigma^2 + \lambda^2}
%                                                    \label{eq:one-sided-chebyshev}
% \end{align}
% %
% 
% To stay in safe region with high probability $1-\delta$, we want $\Prob(\CBCtwo \le
% 0) \le \delta$.
% So we substitute $\lambda = \mCBCtwo > 0$ in \eqref{eq:one-sided-chebyshev}.
% Note that the left inequality does not
% provide an upper bound on the desired distribution, hence on safety.
% We will explicitly avoid the case of left inequality
% by enforcing $\mCBCtwo > 0$,
% %
% \begin{align}
%   \Prob\left(\CBCtwo  \le 0 \right) 
%     \le \frac{\VCBCtwo }{\VCBCtwo + \mCBCtwo^2} \le \delta & \text{ and } \mCBCtwo > 0
% \end{align}
% %
% Once that is satisfied, then we are in the safe region. So we put the two conditions together to get a deterministic condition,
% %
% \begin{align}
%   \mCBCtwo &\ge \sqrt{\frac{1-\delta}{\delta}\VCBCtwo} \ge 0.
% \end{align}
% %
% 
% The condition enforces hat the CBC condition should be satisfied in mean
% and the standard deviation of the CBC condition should be smaller than the mean
% by a factor of $\sqrt{\frac{1-\delta}{\delta}}$.

==> tex/CBCerror.tex <==
%\subsubsection{Proof of Lemma~\ref{lem:NRcalculation} (The posterior of CBC)}
%\begin{proof}
%\end{proof}

==> tex/KnonwLipshitzsefltriggering.tex <==
%\subsubsection{Proof of Theorem~\ref{ir5o45t!!!} (self-triggered control)}
%\MJ{This can go up.}


==> tex/conditionalprobability.tex <==
\subsubsection{Proof of Theorem~\ref{safty-sampl} (The conditional safety probability)}
%\begin{proof}
Using~\eqref{eq:cbcrelations} and $\widehat{\mbox{CBC}}_k \ge \nu$ we deduce 
\begin{align}
  \mathbb{P}(\mbox{CBC}_k \ge \zeta) = \mathbb{P}(\Pi_k \le \widehat{\mbox{CBC}}_k -\zeta)
  \ge \mathbb{P}(\Pi_k \le \nu -\zeta).
\end{align}
Using Lemma~\ref{lem:NRcalculation}, $\mathbb{P}(\Pi_k \le \nu -\zeta)$ is   a cumulative distribution function (CDF) of Gussain random variable $\Pi_k$ at point $\nu -\zeta$, and the result follows.
%\end{proof}

==> tex/mean-and-variance-of-cbf-2/cbc-2-pendulum.tex <==

\paragraph{Pendulum model}
\begin{align*}
\bfx &= [\theta, \omega]
&
\bfu &= [u]
\\
f(\bfx)  &= \left[\omega, -\frac{g}{l}\sin(\theta)\right]^\top
&
g(\bfx) &= \left[0, \frac{1}{ml} \right]^\top
\\
h(\bfx) &=  \cos(\Delta_{col}) - \cos(\theta - \theta_c)
&
\grad_\bfx h(\bfx) &= \left[ \sin(\theta - \theta_c),  0 \right]^\top
\\
H_{\bfx,\bfx} h(\bfx) &= \begin{bmatrix} 
\cos(\theta - \theta_c) & 0 \\ 0 & 0\end{bmatrix}
\end{align*}

\paragraph{Computing $\CBC$}
\begin{align*}
\E[CBC ](\bfx, \bfu) &= \grad_\bfx h(\bfx)^\top \bfM(\bfx) \ctrlaff + h(\bfx)
\\
                     &=  \left[ \sin(\theta - \theta_c),  0 \right]^\top \bfM_k(\bfx) \ctrlaff + \alpha[\cos(\Delta_{col}) - \cos(\theta - \theta_c)]
\\
\Var[CBC](\bfx, \bfx'; \bfu)
&= \ctrlaff^\top \bfB_k(\bfx, \bfx')\ctrlaff 
A_{11}\sin(\theta - \theta_c)^2
\\
&= (\bfB_k(\bfx, \bfx')_{2,2}u^2 + 2\bfB_k(\bfx, \bfx')_{1,2}u + \bfB_k(\bfx, \bfx')_{1,1})
\bfA_{11}\sin(\theta - \theta_c)^2
\end{align*}

\paragraph{Computing $\CBCtwo$}

Computing $\Lie_f h(\bfx)$
\begin{align*}
 \E[\Lie_f h ](\bfx)   &= \grad h(\bfx)^\top \bfM_k(\bfx)_{:, 1}
 \\
 \Var[\Lie_f h](\bfx, \bfx') &= \bfB_k(\bfx, \bfx')_{1, 1} \grad h(\bfx)^\top \bfA \grad h(\bfx)
 \\
 &=  \bfB_k(\bfx, \bfx')_{1, 1} \bfA_{11}\sin(\theta - \theta_c)^2
 \\
 \cov(\Lie_f h, F(\bfx)\ctrlaff)
 &= B_k(\bfx, \bfx')_{1,:}^\top \ctrlaff \grad h(\bfx)^\top \bfA
 \\
 &= B_k(\bfx, \bfx')_{1,:} \ctrlaff \bfA_{1, :} \sin(\theta - \theta_c)
\end{align*}

Computing $\grad \Lie_f h(\bfx)$
\begin{align*}
 \E[\grad \Lie_f h ](\bfx)   
 &= H_{\bfx,\bfx} h(\bfx)^\top \bfM_k(\bfx)_{:, 1}
 + J^\top_\bfx \bfM_k(\bfx)_{:, 1} \grad h(\bfx)
 \\
 &= [ \cos(\theta - \theta_c) \bfM_k(\bfx)_{1,1},  0]^\top
 + J^\top_\bfx \bfM_{:,1} [\sin(\theta - \theta_c), 0]^\top
 \\
 \Var[\grad \Lie_f h](\bfx, \bfx') &= H_{\bfx,\bfx'}\bfB_k(\bfx, \bfx')_{1, 1} \grad h(\bfx)^\top \bfA \grad h(\bfx)
 \\
 &+ \grad h(\bfx')\bfA^\top H_{xx} h(\bfx) \grad_\bfx \bfB_k(\bfx, \bfx')_{1,1}
 \\
 &+ \grad_\bfx \bfB_k(\bfx, \bfx')_{1,1} \grad h(\bfx)^\top \bfA \grad h(\bfx)
 \\
 &+ \bfB_k(\bfx, \bfx')_{1,1}H_{x,x} h(\bfx) \bfA H_{x,x} h(\bfx')
 \\
 &\qquad
 \\
 &=  H_{x,x} \bfB_k(\bfx, \bfx')_{1, 1} \bfA_{11}\sin(\theta - \theta_c)^2
 \\
 &+ \grad_{\bfx} \bfB_k(\bfx, \bfx')_{1, 1} \bfA_{11} [2 \sin(\theta - \theta_c)\cos(\theta - \theta_c), 0]^\top
 \\
 &+ \bfB_k(\bfx, \bfx')_{1, 1} \bfA_{11} \begin{bmatrix}  2 \cos(\theta - \theta_c)^2 - 2 \sin(\theta - \theta_c)^2 & 0 \\ 0 & 0\end{bmatrix}
 \\
 \cov(\grad \Lie_f h, F(\bfx)\ctrlaff)
 &= B_k(\bfx, \bfx')_{1,:}^\top \ctrlaff \grad h(\bfx)^\top \bfA
 \\
 &= B_k(\bfx, \bfx')_{1,:} \ctrlaff \bfA_{1, :} \sin(\theta - \theta_c)
\end{align*}

==> tex/mean-and-variance-of-cbf-2/cbf-2-affine-quadratic.tex <==
\subsubsection{Mean is affine and Variance is quadratic}
\label{proof:mean-affine-var-quadratic}
Next we want to see if the mean and variance are quadratic or higher in $\bfu$.
Expanding each term in $\mCBCtwo$.

%
\begin{align}
  \bar{\bfz}(\bfx; \bfu)\Lambda \bar{\bfz}(\bfx; \bfu)
  &= \grad \tdLie_f h(\bfx)^\top \mDynAffs(\bfx)\ctrlaff
  \\
  \tr(\Lambda \Sigma_\bfz(\bfx, \bfx; \bfu))
  &= \tr(\cov(\grad \tdLie_fh(\bfx), \hDynAff(\bfx)\ctrlaff))
  \\
  &= \tr(\grad_\bfx \ktdfbfu(\bfx,\bfx')\ctrlaff\grad h(\bfx)^\top 
    + \ktdfbfu(\bfx,\bfx')\ctrlaff H_{xx} h(\bfx)^\top)
  \\
  \bfd(\bfx; \bfu)^\top\bar{\bfz}(\bfx; \bfu)
  &= 
    \grad \bLie_{f} h(\bfx)^\top \mDynAffs(\bfx)\ctrlaff
    + \overline{\grad \tdLie_f h(\bfx)}^\top [ \barf(\bfx) + \barg(\bfx)\bfu ] 
    + K_{\alpha,2}\overline{\tdLie_f h(\bfx)}
\end{align}%
% 
Hence, the expectation $\mCBCtwo$ is actually control-affine,
%
\begin{multline}
\mCBCtwo = \grad \tdLie_f h(\bfx)^\top \mDynAffs(\bfx)\ctrlaff
\\
    + \grad_\bfx \ktdfbfu(\bfx,\bfx')\ctrlaff\grad h(\bfx)^\top 
    + \ktdfbfu(\bfx,\bfx')\ctrlaff H_{xx} h(\bfx)^\top
    \\
    + \grad \bLie_{f} h(\bfx)^\top \mDynAffs(\bfx)\ctrlaff
    + \overline{\grad \tdLie_f h(\bfx)}^\top [ \barf(\bfx) + \barg(\bfx)\bfu ] 
    + K_{\alpha,2}\overline{\tdLie_f h(\bfx)}
    \\
+ \grad \bLie_{f} h(\bfx)^\top[ \barf(\bfx) + \barg(\bfx)\bfu ]
+ K_{\alpha,1} h(\bfx) + K_{\alpha,2} \bLie_{f} h(\bfx)
\end{multline}%
% 

Next we expand each term in $\VCBCtwo$ to see if it is quadratic in control $\bfu$.
%
\begin{align}
  2\tr(\Lambda \Sigma_\bfz(\bfx, \bfx; \bfu))^2
  &= \tr(\cov(\grad \tdLie_fh(\bfx), \hDynAff(\bfx)\ctrlaff))
\end{align}
\begin{align}
  \Lambda \Sigma_\bfz(\bfx, \bfx; \bfu) \Lambda
  &=
    \begin{bmatrix}
      0.5\cov(\grad \tdLie_f h(\bfx), \hDynAff(\bfx)\ctrlaff)
      &  0.5\ctrlaff^\top \ktdbfu(\bfx, \bfx')\ctrlaff
      & 0.5 \cov(\tdLie_f h(\bfx), \tdbff(\bfx'; \bfu))
      \\
      0.5K_{\grad \tdLie_f h}(\bfx, \bfx')
      & 0.5\cov(\grad \tdLie_f h(\bfx), \tdbff(\bfx'; \bfu))
      & 0.5\cov(\grad \tdLie_f h(\bfx), \tdLie_f h(\bfx))
    \\
    0 & 0 & 0
  \end{bmatrix} \Lambda
  \nonumber\\
  &=
    \begin{bmatrix}
      0.25\ctrlaff^\top \ktdbfu(\bfx, \bfx')\ctrlaff
      & 0.25\cov(\grad \tdLie_f h(\bfx), \hDynAff(\bfx)\ctrlaff)
      & 0
      \\
      0.25\cov(\grad \tdLie_f h(\bfx), \tdbff(\bfx'; \bfu))
      & 0.25K_{\grad \tdLie_f h}(\bfx, \bfx')
      & 0
    \\
    0 & 0 & 0
  \end{bmatrix}
  \\
  4\bar{\bfz}(\bfx; \bfu)^\top \Lambda
  \Sigma_\bfz&(\bfx, \bfx; \bfu) \Lambda \bar{\bfz}(\bfx; \bfu)
               = 
\grad \tdLie_f h(\bfx)^\top \ctrlaff^\top \ktdbfu(\bfx, \bfx')\ctrlaff \grad \tdLie_f h(\bfx)
  \nonumber\\
  &
    + 2\grad \tdLie_f h(\bfx)^\top \cov(\grad \tdLie_f h(\bfx), \hDynAff(\bfx)\ctrlaff)  \hDynAff(\bfx)\ctrlaff
  \nonumber\\
  &
    +  \ctrlaff^\top\hDynAff(\bfx)^\top K_{\grad \tdLie_f h}(\bfx, \bfx') \hDynAff(\bfx)\ctrlaff
\end{align}
\begin{align}
  \bfd(\bfx; \bfu)^\top
  \Sigma_\bfz&(\bfx, \bfx; \bfu) \bfd(\bfx; \bfu)
               =
               (\barf(\bfx) + \barg(\bfx)\bfu)^\top K_{\grad \tdLie_f h}(\bfx, \bfx')(\barf(\bfx) + \barg(\bfx)\bfu)
  \nonumber\\
             &+ \grad \bLie_f h(\bfx)^\top\ctrlaff^\top \ktdbfu(\bfx, \bfx')\ctrlaff \grad \bLie_f h(\bfx)
  \nonumber\\
  &+ K_{\alpha,2} \knl_{\tdLie_f h}(\bfx, \bfx') K_{\alpha,2}
  \nonumber\\
  &+ 2(\barf(\bfx) + \barg(\bfx)\bfu)^\top \cov(\grad \tdLie_f h(\bfx), \tdbff(\bfx'; \bfu))^\top \grad \bLie_f h(\bfx)
  \nonumber\\
  &+ 2(\barf(\bfx) + \barg(\bfx)\bfu)^\top \cov(\grad \tdLie_f h(\bfx), \tdLie_f h(\bfx))  K_{\alpha,2}
  \nonumber\\
  &+ 2\grad \bLie_f h(\bfx)^\top\ctrlaff^\top\cov(\tdLie_f h(\bfx), \tdbff(\bfx'; \bfu))^\top    K_{\alpha,2}
\end{align}%
% 
%
\begin{align}
  4 \bfd(\bfx; \bfu)^\top
  & \Sigma_\bfz(\bfx, \bfx; \bfu) \Lambda \bar{\bfz}(\bfx; \bfu)
  = 2 \bfd(\bfx; \bfu)
  \begin{bmatrix}
    \cov(\grad \tdLie_f h(\bfx), \tdbff(\bfx'; \bfu))
    & K_{\grad \tdLie_f h}(\bfx, \bfx')
    & 0 \\
    \ctrlaff^\top \ktdbfu(\bfx, \bfx')\ctrlaff
    & \cov(\grad \tdLie_f h(\bfx), \tdbff(\bfx'; \bfu))^\top
    &  0 \\
    \cov(\grad \tdLie_f h(\bfx), \tdLie_f h(\bfx))^\top
    & \cov(\tdLie_f h(\bfx), \tdbff(\bfx'; \bfu))
    &  0
  \end{bmatrix}
      \bar{\bfz}(\bfx; \bfu)
  \nonumber\\
  &= (\barf(\bfx) + \barg(\bfx)\bfu)^\top
    \cov(\grad \tdLie_f h(\bfx), \tdbff(\bfx'; \bfu))
    \grad \tdLie_f h(\bfx)
    \nonumber\\
  &+ (\barf(\bfx) + \barg(\bfx)\bfu)^\top
  K_{\grad \tdLie_f h}(\bfx, \bfx')
  \hDynAff(\bfx)\ctrlaff
    \nonumber\\
  &+ \grad \bLie_f h(\bfx)^\top
    \ctrlaff^\top \ktdbfu(\bfx, \bfx')\ctrlaff
    \grad \tdLie_f h(\bfx)^\top
    \nonumber\\
    &+ \grad \bLie_f h(\bfx)^\top
      \cov(\grad \tdLie_f h(\bfx), \tdbff(\bfx'; \bfu))^\top
      \hDynAff(\bfx)\ctrlaff
    \nonumber\\
    &+ K_{\alpha,2}
    \cov(\grad \tdLie_f h(\bfx), \tdLie_f h(\bfx))^\top
    \grad \tdLie_f h(\bfx)
    \nonumber\\
  &+ K_{\alpha,2}\cov(\tdLie_f h(\bfx), \tdbff(\bfx'; \bfu))
      \hDynAff(\bfx)\ctrlaff
\end{align}%
% 
Since all the terms at most quadratic in $\bfu$, this means that $\VCBCtwo$ is
quadratic in $\bfu$.

==> tex/mean-and-variance-of-cbf-2/positive-definiteness.tex <==
\subsubsection{Is the deterministic condition positive-definite?}
For a relative degree 2 system, we can write $\CBCtwo$ as 


==> tex/mean-and-variance-of-cbf-2/proof-mvg-cov.tex <==
%\subsubsection{Matrix Variate Gaussian Covariance (Lemma~\ref{lemma:product-mvg})}
%\label{proof:mvg-cov}

Without loss of generality assume $\bfX$ and $\bfY$ have mean $\mathbf{0}$.
Let $\bfY = [ \bfy_1, \dots, \bfy_l ]$ and $\bfX = [ \bfx_1, \dots, \bfx_n]$.
%
\begin{align}
  \cov(\vect(\bfX), \vect(\bfY))
  = \E[\vect(\bfX)\vect(\bfY)^\top] = \bfB \otimes \bfA
\end{align}%
% 
Multiply both sides by $\bfI_n \otimes \bfC$, we get
\begin{align}
    \E[(\bfI_n \otimes \bfC)\vect(\bfX)\vect(\bfY)^\top] = (\bfI_n \otimes \bfC)(\bfB \otimes \bfA)
\end{align}
Applying $(\bfP \otimes \bfQ)\vect(\bfR) = \vect(\bfQ\bfR\bfP^\top)$ to the left hand side and $(\bfP \otimes \bfQ)(\bfR \otimes \bfS) = \bfP\bfR \otimes \bfQ\bfS$ to the right hand side, we get
\begin{equation}
\begin{aligned}
    \E[\vect(\bfC\bfX\bfI_n^\top)\vect(\bfY)^\top] = (\bfI_n\bfB \otimes \bfC\bfA)
    \\
    = \cov(\vect(\bfC\bfX),\vect(\bfY)) = \bfB \otimes \bfC\bfA
\end{aligned}
\end{equation}

Second part can be proved by noticing that,
%
\begin{equation}
\begin{aligned}
\cov(\vect(\bfX^\top), \vect(\bfY^\top)) &= \bfA \otimes \bfB
  \\
\implies \cov(\vect(\bfD^\top \bfX^\top),\vect(\bfY^\top)) &= \bfA \otimes \bfD^\top \bfB
  \\
\implies \cov(\vect(\bfX \bfD),\vect(\bfY)) &= \bfD^\top \bfB \otimes \bfA
\end{aligned}%
\end{equation}
% 

==> tex/mean-and-variance-of-cbf-2/sanity-check.tex <==
\subsubsection{Sanity check for matrix calculus \eqref{eq:grad-of-lie-h}}
\label{proof:grad-of-lie-h}


%
\begin{align}
  \grad_\bfx \Lie_fh(\bfx)^\top &= \grad_\bfx [ \grad_\bfx h(\bfx)^\top f(\bfx) ]
                             %
  =\begin{bmatrix} \frac{\p \Lie_fh(\bfx)}{\p x_1}
    &\dots & \frac{\p \Lie_fh(\bfx)}{\p x_n}
    \end{bmatrix}
      %
\end{align}%
% 

Computing derivatives element wise,
%
\begin{align}
  \Lie_fh(\bfx) &= \grad_\bfx h(\bfx)^\top f(\bfx) = f_1(\bfx) \frac{\p h}{\p x_1}
  + \dots + f_n(\bfx) \frac{\p h}{\p x_n}
  \\
  \grad_\bfx \Lie_fh(\bfx) &= \begin{bmatrix}
    \frac{\p f_1}{\p x_1} \frac{\p h}{\p x_1}
    + f_1(\bfx) \frac{\p^2 h}{\p x_1 \p x_1}
    + \dots
    + \frac{\p f_n}{\p x_1} \frac{\p h}{\p x_n}
    + f_n(\bfx) \frac{\p^2 h}{\p x_1 \p x_n}
    \\
    \vdots
    \\
    \frac{\p f_1}{\p x_n} \frac{\p h}{\p x_1}
    + f_1(\bfx) \frac{\p^2 h}{\p x_n \p x_1}
    \dots
    + \frac{\p f_n}{\p x_n} \frac{\p h}{\p x_n}
    + f_n(\bfx) \frac{\p^2 h}{\p x_n \p x_n}
    \end{bmatrix}
  \label{eq:sanity-elementwise}
\end{align}%
% 

Computing derivatives by matrix calculus,
%
\begin{align}
  \grad_\bfx \Lie_fh(\bfx) &= \grad_\bfx [\grad_\bfx h(\bfx)^\top f(\bfx)]
                       = H_{xx}h(\bfx) f(\bfx)  + J_x^\top f(\bfx)\grad_\bfx h(\bfx)
  \\
               &= \begin{bmatrix}
                 f_1(\bfx)\frac{\p^2 h}{\p x_1 \p x_1}
                 + \dots + f_n(\bfx)\frac{\p^2 h}{\p x_1 \p x_n}
                 \\ \vdots \\
                 f_1(\bfx)\frac{\p^2 h}{\p x_n \p x_1}
                 + \dots + f_n(\bfx)\frac{\p^2 h}{\p x_n \p x_n}
               \end{bmatrix}
                   +
                   \begin{bmatrix}
                     \frac{\p h}{\p x_1}\frac{\p f_1}{\p x_1}
                     + \dots + \frac{\p h}{\p x_n}\frac{\p f_n}{\p x_1}
                     \\ \vdots \\
                     \frac{\p h}{\p x_1}\frac{\p f_1}{\p x_n}
                     + \dots + \frac{\p h}{\p x_n}\frac{\p f_n}{\p x_n}
                   \end{bmatrix}
  \\
               &= \begin{bmatrix}
                 f_1(\bfx)\frac{\p^2 h}{\p x_1 \p x_1}
                 + f_n(\bfx)\frac{\p^2 h}{\p x_1 \p x_n}
                 + \dots + \frac{\p h}{\p x_1}\frac{\p f_1}{\p x_1}
                 + \frac{\p h}{\p x_n}\frac{\p f_n}{\p x_1}
                 \\ \vdots \\
                 f_1(\bfx)\frac{\p^2 h}{\p x_n \p x_1}
                 + f_n(\bfx)\frac{\p^2 h}{\p x_n \p x_n}
                 + \dots + \frac{\p h}{\p x_1}\frac{\p f_1}{\p x_n}
                 + \frac{\p h}{\p x_n}\frac{\p f_n}{\p x_n}
               \end{bmatrix}
  \label{eq:sanity-matrix-calculus}
\end{align}%
% 
Terms \eqref{eq:sanity-matrix-calculus} and \eqref{eq:sanity-elementwise} are
the same.
\hfill $\blacksquare $

==> tex/mean-and-variance-of-cbf-r.tex <==
Let the kernel of the dynamics $f(\bfx)$ be an exponential kernel. It can be
shown that the double derivative of the exponential kernel is the kernel itself
with a scale factor

\begin{lemma}[Double derivative of exponential kernel]
  If $\knl(\bfx_1, \bfx_2) = \exp(-0.5(\bfx_1 - \bfx_2)\Sigma^{-1}(\bfx_1 -
  \bfx_2))$, then
  \begin{align}
    \frac{\partial^2 \knl(\bfx_1, \bfx_2)}
    {\partial \bfx_1 \partial \bfx_2} \Big|_{\bfx_1 = \bfx_2}
    &= \Sigma^{-1} \knl(\bfx_1, \bfx_2)
  \end{align}%
\end{lemma}%
%

Let the Control Barrier Function $h(\bfx)$ be of degree $r$, i.e.
$\Lie_g^{(r-1)} h(\bfx) = 0$, then the $(r-1)$th Lie derivative of $f(\bfx)$ is
given by the following recursive formula

%
\begin{align}
  \Lie_f^{(1)} h(\bfx) &= \grad_\bfx [h(\bfx)]^\top f(\bfx)
  \\
  \Lie_f^{(i+1)} h(\bfx) &= \grad_\bfx [\Lie_f^{(i)} h(\bfx)]^\top f(\bfx) \qquad \forall i \in \{ 1, \dots, r-1 \}
\end{align}%
%
The above computation can be written visualized in terms of a graph as shown in
Figure~\ref{fig:mean-and-variance-of-cbf-r-diagram}.
Note that in the graph there are only two operators, the gradient and the dot
product.

\begin{figure}
\input{tex/mean-and-variance-of-cbf-r-diagram.tex}
\caption{Computation graph for higher order Lie derivative}
\label{fig:mean-and-variance-of-cbf-r-diagram}
\end{figure}


We have already shown that $\Lie_f^{(2)} h(\bfx)$ is a Gaussian process whose
mean and variance can be analytically computed. We focus our attention on
$\Lie_f^{(3)} h(\bfx)$.

%
\begin{align}
  \Lie_f^{(3)} h(\bfx) = \grad_\bfx [\Lie_f^{(2)} h(\bfx)]^\top f(\bfx)
\end{align}%
%

By Lemma~\ref{lemma:differentiating-gp}, the gradient of a GP $\grad_\bfx \Lie_f^{(2)}
h(\bfx)$ is also a Gaussian Process.
We again write $\grad_\bfx [\Lie_f^{(2)} h(\bfx)]^\top f(\bfx)$ in a quadratic form,

%
\begin{align}
  \Lie_f^{(3)} h(\bfx)
  &=
    \begin{bmatrix}
      \grad_\bfx [\Lie_f^{(2)} h(\bfx)] \\
      f(\bfx)
 \end{bmatrix}^\top
\begin{bmatrix}
  0.5 & 0 \\
  0 & 0.5
\end{bmatrix}
    \underbrace{\begin{bmatrix}
      \grad_\bfx [\Lie_f^{(2)} h(\bfx)] \\
      f(\bfx)
 \end{bmatrix}}_{\triangleq z(\bfx)}
\end{align}
%

Also let the variance of $z(\bfx)$ be $\Var(z(\bfx))$. Let the Cholesky
factorization of $\Var(z(\bfx))$ be $A(\bfx)A(\bfx)^\top \triangleq \Var(z(\bfx))$.
Then $w(\bfx) \triangleq A^{-1}(\bfx) (z(\bfx)-\E[z(\bfx)]) $ has the variance as identity:
%
\begin{align}
  \Var(w(\bfx)) \triangleq \E[w(\bfx)w(\bfx)^\top]
  = \E[ A^{-1}(\bfx) z(\bfx) z(\bfx)^\top A^{-\top}(\bfx) ]
  = A^{-1}(\bfx) \Var(z(\bfx)) A^{-\top}(\bfx) = I.
\end{align}%
%

So $\Lie_f^{(3)} h(\bfx)$ can be written in terms of $w(\bfx)$,
%
\begin{align}
  \Lie_f^{(3)} h(\bfx)
  &= w(\bfx)^\top
  \underbrace{A^\top(\bfx)
  \begin{bmatrix} 0 & 0.5 \\ 0.5 & 0 \end{bmatrix}
                                 A(\bfx)
                                 }_{\Lambda(\bfx)}
                                 w(\bfx)
                                 + 2 w(\bfx)^\top A(\bfx)\E[z(\bfx)] 
                                 + \E[z(\bfx)]^2
  \\
  &= w(\bfx)^\top \Lambda(\bfx) w(\bfx)
  + 2 w(\bfx)^\top A(\bfx)\E[z(\bfx)] 
  + \E[z(\bfx)]^2
\end{align}
%

Note that $w(\bfx)$ is a zero-mean unit variance Gaussian random vector with
independent coordinates. Next we recall a recent extension of Hansen-Wright
inequality~\cite{gotze2019concentration},

%
\begin{definition}[Orclitz norm]
  The Orclitz norm $\|X\|_{\Psi_\alpha}$ of a random variable $X$ is defined as:
  %
  \begin{align}
    \|X\|_{\Psi_\alpha} \triangleq \inf\left\{
    t \ge 0 : \E \exp\left(\frac{\|X\|^\alpha}{t^\alpha} \right) \le 2
    \right\},
  \end{align}
  %
  where $\inf \phi = \infty$.
  Note that Orclitz norm is only a norm for $\alpha > 1$ to satisfy the
  triangle inequality.
\end{definition}

%
\begin{theorem}[Concentration of Sub-$\alpha$ exponential RV \citep{gotze2019concentration}]
  \label{thm:sub-alpha-exp-rv}
  Let $X_1, \dots, X_n$ be independent random variables satisfying $\E[X_i] = 0,
  \E[X_i^2] = \sigma_i^2, \|X_i\|_{\Psi_\alpha} \le M$ for some $\alpha \in (0,
  1] \cup \{2\}$, and $A$ be a symmetric $n \times n$ matrix.

  For any $t > 0$ we
  have,
  \begin{align}
    P\left(
    \left|
    X^\top A X - \tr( \diag(\{\sigma_i^2\}_{i=1}^n) A)
    \right| \ge t
    \right)
  \le 2 \exp\left(-\frac{1}{C}
    \min\left( \frac{t^2}{M^4 \|A\|_{HS}^2},
      \left(\frac{t}{M^2 \|A\|_{op}} \right)^{\frac{\alpha}{2}}
      \right)
    \right).
    \end{align}
\end{theorem}
%

For our case, $X_i = w(\bfx)_i$ and all $\sigma_i = 1$. Also the Orclitz norm
$\|X_i\|_{\Psi_\alpha}$ for $\alpha = 2$ exists for sub-Gaussian random
variables.
Since, $w(\bfx)_i$ is Gaussian random variables, hence
$\|w(\bfx)_i\|_{\Psi_\alpha}$ exists with $\alpha = 2$.

Applying Theorem~\ref{thm:sub-alpha-exp-rv} to $w(\bfx)^\top \Lambda(\bfx)
w(\bfx)$ with $\alpha = 2$, we get,
%
\begin{align}
  P\left(\left| w(\bfx)^\top \Lambda(\bfx) w(\bfx) - \tr(\Lambda(\bfx)) \right| \ge t \right)
  \le 2 \exp\left(-\frac{1}{C}
    \min\left( \frac{t^2}{M^4 \|\Lambda(\bfx)\|_{HS}^2},
      \frac{t}{M^2 \|\Lambda(\bfx)\|_{op}}
      \right)
    \right).
\end{align}

We already know that $w(\bfx)$ being a Gaussian random vector,
%
\begin{align}
  P\left(\left| w(\bfx)^\top A(\bfx) E[z(\bfx)] \right| \ge t \right)
  \le c \exp\left(-\frac{t^2}{C} \right)
\end{align}
%

We can conclude that
$\Lie^{(3)}_f h(\bfx)$ is sub-exponential random vector,
%
\begin{align}
  P\left( \left| \Lie^{(3)}_f h(\bfx) - \E[\Lie^{(3)}_f h(\bfx)] \right| \ge t \right)
  \le C \exp\left( -\frac{t}{c} \right).
\end{align}%
% 

We have already seen that derivative of the random process with exponential
kernel does not change the the tail bounds of the random process.

For arbitrary $r \ge 2$th Lie derivative, we have
%
\begin{align}
  P\left( \left| \Lie^{(r)}_f h(\bfx)
  - \E[\Lie^{(r)}_f h(\bfx)] \right| \ge t \right)
  \le C \exp\left( -\frac{t^{\frac{2}{r-1}}}{c} \right).
\end{align}
  

==> tex/note11.tex <==
We use bold faced letters for vectors ($\bfx$), capital letters for matrices
($\bfX$), caligraphic capital letters for sets ($\calC$) and
underline letters $\underline{\bfu} = [1, \bfu^\top]^\top$ for homogeneous coordinates. We use $\otimes$ for the Kronecker product, and $\erf$ for the Gauss error
function. $\partial \mathcal{C}$ denotes the boundry of the set $\mathcal{C}$.
Let $\textit{vec}(\bfX) \in \mathbb{R}^{nm}$ be the vectorization of $\bfX \in
\R^{n \times m}$, obtained by stacking the columns of $\bfX$. For the functions $h : \real \rightarrow
\real^n$  and $f : \real^n \rightarrow
\real^n$ the Hessian and Jacobian are defined as follows
%
%For a function 
%Let  of $h(\bfx)$  $J_x f(\bfx)$ of
%$f(\bfx)$ be defined as,
\newcommand{\p}{\partial}
%
\begin{align}
  \calH_{xx} h(\bfx) &\triangleq \begin{bmatrix}
    \frac{\p h}{\p x_1 \p x_1} & \dots & \frac{\p h}{\p x_1 \p x_n}
    \\
    \vdots & & \vdots
    \\
    \frac{\p h}{\p x_n \p x_1} & \dots & \frac{\p h}{\p x_n \p x_n}
  \end{bmatrix},
                                       \\%&
    \calJ_\bfx f(\bfx) &\triangleq \begin{bmatrix}
    \frac{\p f_1}{\p x_1} & \dots & \frac{\p f_1}{\p x_n}
    \\
    \vdots & & \vdots
    \\
    \frac{\p f_n}{\p x_1} & \dots & \frac{\p f_n}{\p x_n}
    \end{bmatrix}.
\end{align}%
% 
%The following parameters are useful for our analysis in Sec.~\ref{sec:exp-cbf-rel-deg-2} 



==> tex/old/Inference.tex <==

\section{Matrix Variate Gaussian Process Regression of System Dynamics}
\label{learningsec:13452}
In this section we deal with the Problem~\ref{prb:learning} by developing an efficient GP framework for control-affine systems. More precisely, we use the matrix variate Gaussian (MVG) distribution~\cite{StructuredPBP} to characterize posteriors over $f$ and $g$. These posteriors will be used determine a posterior for CBC, later in Section~\ref{sec:unknowndynamics}.
\NA{I would emphasize the novelty of this section by naming and presenting it as ``Matrix Variate Gaussian Process Regression of Nonlinear Control-Affine System Dynamics''.}
%We use different methods for supervised learning Gaussian process, neural networks, Bayesian neural networks approximation (droup out), Bayesian neural networks: Deterministic Variational Inference~\cite{wu2018deterministic}.
%Let $z=(x^{\top},u^{\top})^{\top}$.
%We assume $\bar{g}u+\bar{f}=\sum_{i=1}^{\infty} \alpha_i$
%\bibliographystyle{plainnat}
%\def\localbib{\string~/wrk/group-bib/shared}
%IfFileExists{\localbib.bib}{
%\bibliography{\localbib,main_filtered}}{
%\bibliography{main_filtered}}
%The system of \eqref{eq:system_dyanmics} can written as,
%
%\begin{align}
  %\underbrace{\stdt - \barf(\state) - \barg(\state)\bfu}_{\tddotx :=} &= \tdf(\state) +  \tdg(\state) \ctrl,
  %& 
%  \bfx &= \underbrace{\begin{bmatrix}
%            f(\state)&  g(\state)
%          \end{bmatrix}}_{\dynAff(\state) :=}
 %                            \underbrace{\begin{bmatrix}1\\
                             %\ctrl\end{bmatrix}}_{\ctrlaff :=},
  %&
  %\stdt &= \dynAff(\state)\ctrlaff.
   %       \label{eq:affine-gp-cont}
%\end{align}%
% 
%We assume $\vect(\dynAff)$ to be a Gaussian process $\vect(\dynAff) \sim \GP(0,
%\kDA)$, where $\kDA$ is the vector kernel function $\kDA: \StateSp \times
%\StateSp \mapsto \R^{n(1+m) \times (1+m)n}$.
As in Coregionalization models~\cite{alvarez2012kernels} we assume the kernel of GP distribution over $\vect(F(\bfx))$, $\bfK_k(\bfx,\bfx'): \R^{n} \times
\R^{n} \mapsto \R^{n(1+m) \times (1+m)n}$, can factorized into a state dependent component $\knl_k(\state, \state')$ and a
output dimensions dependent covariance matrix $\KDA_k \in \R^{n(1+m) \times (1+m)n}$,
%
\begin{align}
\bfK_k(\bfx,\bfx') = \KDA_k \knl_k(\state, \state').
\end{align}%
% 

We note that Gaussian process $\dynAff$ is a matrix variate function and $\KDA$
can be  large matrix for high dimensional systems.
Learning the $(1+m)^2n^2$ parameters of kernel $\KDA$ requires large amount of
training data. To avoid the need of large training data, we use MVG distributions. The definition of MVG and some related results that we used in this section is detailed in
appendix~\ref{sec:MGVresutls2} for completeness. 
%\subsubsection{Matrix Variate Gaussian Process}

In line with MVG distributions,
we let 
%we define the matrix function 
%$\dynAff$ 
%\StateSp \rightarrow \R^{n \times (1+m)}$ 
%to be a MVG Process 
$F \sim \mathcal{MGP}(\bfM, \bfA, \bfB, \knl)$  with parameters
$\bfM = 0_{n \times (1+m)}$, $\bfA \in \R^{n \times n}$, 
$\bfB \in \R^{(1+m) \times (1+m)}$ and 
$\knl : \StateSp \times \StateSp \rightarrow \R^+$ is positive definite kernel,
   if 
%
\begin{align}
  \vect(\dynAff) &\sim \mathcal{GP}(\mathbf{0}, \bfK)
  &\text{where }   \bfK(\state, \state') = \KDA \knl(\state, \state') = \bfB \otimes \bfA \knl(\state, \state').
\end{align}%
% 

For training data samples, 
$\StDat_{1:k}$, let corresponding kernel
matrix be
 $\KDat := [\knl(\state_i,\state_j)]_{i=1,j=1}^{k,k}$ ,
and corresponding function values  be
$\dynAffDat(\StDat_{1:k}) := [\dynAff(\state_1), \dots, \dynAff(\state_k)] \in \R^{n \times k(1+m) }$.
An MVG Process evaluated over samples yields an MVG distribution,
%
\begin{align}
  \dynAffDat(\StDat) &\sim \mathcal{MN}(\mathbf{0}, \bfA, \KDat \otimes \bfB).
\end{align}%
% 

Let the training target data be denoted as $\StDtDat_{1:k} \in \R^{n \times k}$, and
$\CtDat_{1:k} := \diag(\ctrlaff_1, \dots, \ctrlaff_k) \in \R^{k(1+m) \times k}$.
We want to find out the function value $\dynAff(\state_*)$ at the
given test state $\state_*$.
Since $\CtDat$ is deterministic, the covariance functions of $\StDtDat_{1:k} = \dynAffDat(\StDat_{1:k}) \CtDat_{1:k}$ and $\dynAff(\state_*)$ can be written in terms of
$\KDat \otimes \bfB$, $\bfA$ and $\CtDat_{1:k}$,
%
\begin{align}
  \KDat_{\StDtDat_{1:k}}
  &:= \cov(\vect(\dynAffDat(\StDat_{1:k}) \CtDat_{1:k}),
                     \vect(\dynAffDat(\StDat_{1:k}) \CtDat_{1:k}))
                     = [ \CtDat_{1:k}^\top [ \KDat \otimes \bfB ] \CtDat_{1:k} ] \otimes \bfA
  %\\
  %&= [\knl(\bfx_i, \bfx_j)\ctrlaff_i^\top B \ctrlaff_j]_{i=1,j=1}^{k,k}  \otimes \bfA
  \\
  \kDat_{\StDtDat,*} &:= \cov(\vect(\dynAffDat(\StDat_{1:k}) \CtDat_{1:k}),
                       \vect(\dynAffDat(\state_*)))
           = [ \CtDat_{1:k}^\top [ \kDat_* \otimes \bfB ]] \otimes \bfA
  %\\
  %&= [\knl(\bfx_i, \bfx_j)\ctrlaff_i^\top B]_{i=1,j=1}^{k,k}  \otimes \bfA
  \\
  \kDat_{\dynAff_*} &:= \cov(\vect(\dynAffDat(\state_*)), \vect(\dynAffDat(\state_*)))
              = \knl(\state_*, \state_*)\bfB \otimes \bfA,
\end{align}%
% 
where $\kDat_{*} := [k(\bfx_*,\bfx_i)]_{i=1}^k$.
The train data and test data are jointly Gaussian,
%
\begin{align}
  \begin{bmatrix}
    \vect(\StDtDat_{1:k})
    \\
    \vect(\dynAff(\state_*))
  \end{bmatrix}
  \sim
  \N \left(\begin{bmatrix} \mathbf{0} \\ \mathbf{0} \end{bmatrix},
  \begin{bmatrix}
    \KDat_{\StDtDat }
    & 
    \kDat_{\StDtDat,*}
    \\
    \kDat_{\StDtDat,*}^\top
    & \kDat_{\dynAff_*}
  \end{bmatrix}
  \right).
\label{BI:GP232w}
\end{align}%
% 

Then the posterior Gaussian distribution $\vect(\dynAff^*_k(\state_*)) :=
\vect(\dynAff(\state_*)) | \state_*, \StDtDat_{1:k}, \StDat_{1:k}, \CtDat_{1:k}$ is given by,
%
\begin{align}
  \vect(\dynAff^*_k(\state_*))
  %\\
  \sim \N(
  \kDat^\top_{\StDtDat,*} \KDat_{\StDtDat}^{-1}\vect(\StDtDat_{1:k}), 
            \kDat_{\dynAff_*} - \kDat^\top_{\StDtDat,*} \KDat_{\StDtDat}^{-1} \kDat_{\StDtDat,*}).
\end{align}%
% 

The above distributions can be also written (see
Appendix~\ref{proof:matrix-variate-gp}) as an MVG distribution by
factorizing the covariance as a Kronecker product,
%
\newcommand{\mDynAffs}{\bar{\dynAff}^*_k}
\newcommand{\bfBs}{\bfB^*_k}
\begin{align}
  \dynAff^*_k(\state_*)
  %\\
  &\sim \mathcal{MN}(\mDynAffs(\bfx_*), \bfA, \bfBs(\bfx_*, \bfx_*))
  \\
  \text{where }
  \mDynAffs(\bfx_*)
  &:= \StDtDat_{1:k}
  [ \CtDat^\top [ \KDat \otimes \bfB ] \CtDat ]^{-\top}
  \CtDat^\top[ \kDat_* \otimes \bfB ]
  \\
  \bfBs(\bfx_*, \bfx_*)
  &:= \knl(\state_*, \state_*)\bfB
  - 
  [ \kDat_* \otimes \bfB ]^\top \CtDat
  \Bigl( \CtDat^\top [ \KDat \otimes \bfB ] \CtDat \Bigr)^{-1}
  \CtDat^\top [ \kDat_* \otimes \bfB ].
  \label{eq:mvg-posterior}
\end{align}
%

This can be used to compute mean and variance of $f(\bfx) + g(\bfx)\bfu$ for any deterministic $\bfu$ as,
%
\begin{align}
f(\bfx) + g(\bfx)\bfu &\sim \GP(\barf^*_k(\bfx) + \barg^*_k(\bfx)\bfu, \mathcal{K}^*_k)
\\ \text{where }
  \barf^*_k(\bfx) + \barg^*_k(\bfx)\bfu &= \mDynAffs(\bfx) \ctrlaff,
  & \mathcal{K}^*_k(\bfx, \bfx') &= \ctrlaff^\top \bfBs(\bfx, \bfx') \ctrlaff \bfA.
\label{eq:mvg-posterior-bfu-main}
\end{align}

==> tex/old/cbc-3-mean.tex <==
\subsection{Mean of $\CBCthree$}
\label{proof:mean-of-cbc-3}

Recall that $\grad \Lie_{\tdbff}^{(1)} h(\bfx)$ is a Gaussian Process with mean
and variance given by \eqref{eq:mean-var-grad-lie-grad-h-f},
where $\tdbff(\bfx; \bfu) = f(\bfx) + g(\bfx) \bfu$ is the control-affine
dynamics of the system which is assumed to be a Gaussian process in $\bfx$.  
We also have $\cov(\grad \Lie_{\tdbff}^{(1)} h(\bfx), \tdbff(\bfx; \bfu))$.

By definition $\Lie_{\tdbff}^{(2)} h(\bfx) := \grad[
\Lie_{\tdbff}^{(1)}h(\bfx)]^\top \tdbff(\bfx; \bfu)$. 
By using Lemma~\ref{lemma:quadratic-form}, we can compute mean and variance of 
$\Lie_{\tdbff}^{(2)} h(\bfx)$ with $\bfx = [\grad
\Lie_{\tdbff}^{(1)}h(\bfx)^\top, \tdbff(\bfx; \bfu)^\top, \Lie_{\tdbff}^{(1)}
h(\bfx)]^\top$ and $\Lambda = 0.5\begin{bmatrix} 0 & I_n & 0 \\ I_n & 0 & 0
  \\ 0 & 0 & 0\end{bmatrix}$. First note that

%
\begin{align}
  \Sigma \Lambda 
  &= 0.5\begin{bmatrix}
         \Sigma_{12} & 0 & \Sigma_{11} \\
         \Sigma_{22} & 0 & \Sigma_{21} \\
         \Sigma_{32} & 0 & \Sigma_{31}\\
    \end{bmatrix}
  &
    \Lambda \Sigma \Lambda
  & = 0.25\begin{bmatrix}
         \Sigma_{22} & 0 & \Sigma_{21} \\
         \Sigma_{12} & 0 & \Sigma_{11} \\
         0 & 0 & 0
    \end{bmatrix},
\end{align}%
% 
where $\Sigma_{11} = \Var(\grad \Lie_{\tdbff}^{(1)} h(\bfx))$, $\Sigma_{22} = \ktdbfu(\bfx, \bfx')$, $\Sigma_{12} = \Sigma_{21}^\top = \cov(\grad[ \Lie_{\tdbff}^{(1)}h(\bfx)], \tdbff(\bfx; \bfu))$, $\Sigma_{32} = \cov(\Lie_{\tdbff}^{(1)}h(\bfx), \tdbff(\bfx; \bfu))$ and $\Sigma_{31} = \cov(\Lie_{\tdbff}^{(1)}h(\bfx),\grad \Lie_{\tdbff}^{(1)}h(\bfx))$.

%
\begin{align}
    \E[\Lie_{\tdbff}^{(2)} h(\bfx)] 
    &= 
    \E[\grad \Lie_{\tdbff}^{(1)}h(\bfx)]\E[\tdbff(\bfx; \bfu)] + \tr(\cov(\grad[ \Lie_{\tdbff}^{(1)}h(\bfx)], \tdbff(\bfx; \bfu)))
    \\
    \Var[\Lie_{\tdbff}^{(2)} h(\bfx)] 
    &= 
    2\tr(\cov(\grad \Lie_{\tdbff}^{(1)}h(\bfx),\tdbff(\bfx; \bfu)))^2
    + \E[\tdbff(\bfx; \bfu)] \Var(\grad \Lie_{\tdbff}^{(1)} h(\bfx))\E[\tdbff(\bfx; \bfu)]
    \nonumber\\
    &+ \E[\grad \Lie_{\tdbff}^{(1)} h(\bfx)] \ktdbfu(\bfx, \bfx')\E[\grad \Lie_{\tdbff}^{(1)} h(\bfx)]
    \nonumber\\
    &+ 2 \E[\grad \Lie_{\tdbff}^{(1)} h(\bfx)]\cov(\grad \Lie_{\tdbff}^{(1)}h(\bfx),\tdbff(\bfx; \bfu))\E[\tdbff(\bfx; \bfu)]
    \\
    \cov(\Lie_{\tdbff}^{(2)} h(\bfx), \tdbff(\bfx; \bfu)) 
    &= \cov(\grad \Lie_{\tdbff}^{(1)}h(\bfx),\tdbff(\bfx; \bfu))\E[\tdbff(\bfx; \bfu)] + \knl(\bfx, \bfx') \E[\grad \Lie_{\tdbff}^{(1)} h(\bfx)]
    \\
    \cov(\Lie_{\tdbff}^{(2)} h(\bfx), \Lie_{\tdbff}^{(1)}(\bfx))
    &= \cov(\Lie_{\tdbff}^{(1)}h(\bfx),\grad \Lie_{\tdbff}^{(1)}h(\bfx))\E[\tdbff(\bfx; \bfu)] 
    + \cov(\Lie_{\tdbff}^{(1)}h(\bfx), \tdbff(\bfx; \bfu)) \E[\grad \Lie_{\tdbff}^{(1)} h(\bfx)]
\end{align}
%

Note that $\Lie_{\tdbff}^{(2)} h(\bfx)$ is no longer a Gaussian process.
However, both Lemma~\ref{lemma:differentiating-gp} and the expectation part of Lemma~\ref{lemma:quadratic-form}   
are valid for any random process with finite mean and variance.
For this reason the expectation recursive formula is true for arbitrary relative degree $r$,

%
\begin{align}
    \E[\Lie_{\tdbff}^{(r+1)} h(\bfx)] 
    &= 
    \E[\grad \Lie_{\tdbff}^{(r)}h(\bfx)]\E[\tdbff(\bfx; \bfu)] + \tr(\cov(\grad[ \Lie_{\tdbff}^{(r)}h(\bfx)], \tdbff(\bfx; \bfu)))
\end{align}
%
However for $r >= 3$, it is harder to compute $\cov(\grad[ \Lie_{\tdbff}^{(r)}h(\bfx)], \tdbff(\bfx; \bfu))$.
But for $r=3$, we know  $\cov(\grad \Lie_{\tdbff}^{(2)} h(\bfx), \tdbff(\bfx; \bfu)) = \grad \cov(\Lie_{\tdbff}^{(2)} h(\bfx), \tdbff(\bfx; \bfu))$ from Lemma~\ref{lemma:differentiating-gp} which is valid for any random process, not just Gaussian process,
%
\begin{align}
    \E[\Lie_{\tdbff}^{(3)} h(\bfx)] 
    &= 
    \E[\grad \Lie_{\tdbff}^{(2)}h(\bfx)]\E[\tdbff(\bfx; \bfu)] + \tr(\grad\cov( \Lie_{\tdbff}^{(2)}h(\bfx), \tdbff(\bfx; \bfu)))
\end{align}
%

Now $\CBCthree(\bfx; \bfu)$ can be written in terms $\Lie_{\tdbff}^{(3)}
h(\bfx)$,
%
\begin{align}
  \CBCthree(\bfx; \bfu) = \Lie_{\tdbff}^{(3)} h(\bfx)
  + K_\alpha \begin{bmatrix}
    h(\bfx) \\ \Lie_{\tdbff}^{(1)} h(\bfx) \\ \Lie_{\tdbff}^{(2)} h(\bfx) \ge 0
    \end{bmatrix}.
\end{align}%
% 
The expectation of $\CBCthree$ is simply the linear combination of the
expectations,
%
\begin{align}
  \E[\CBCthree(\bfx; \bfu)] = \E[\Lie_{\tdbff}^{(3)} h(\bfx)]
  + K_{\alpha,1} h(\bfx)
  + K_{\alpha,2} \E[\Lie_{\tdbff}^{(1)} h(\bfx)]
  + K_{\alpha,3} \E[\Lie_{\tdbff}^{(2)} h(\bfx)] \ge 0
\end{align}%
% 




==> tex/old/covar-of-jac-of-gp.tex <==
\begin{lemma}[Covariance matrix of Jacobian of Gaussian Process]
  \label{lemma:covar-of-jac-of-gp}
Under assumptions of Lemma~\ref{thm:mean-of-jac-of-gp}, the covariance matrix of
the vectorized $\vect(J_{\bfx_*} f_*(\bfx_*)) \in \R^{ln}$ is given by,
% 
  \begin{align}
    \Cov(\bfj_*, \bfj'_*) &=
    \left[ H_{xx} k(\bfx_*, \bfx'_*)
    - J_{\bfx_*}^\top \bfkx\bfKX J_{\bfx_*}\bfkxp \right] \otimes K^f
  \end{align}%
  % 
  For scalar-valued GP, $K^f = 1$,
% 
  \begin{align}
    \Cov(\bfj_*, \bfj'_*) &= H_{xx} k(\bfx_*, \bfx'_*) - J_{\bfx_*}^\top \bfkx\bfKX J_{\bfx_*}\bfkxp
  \end{align}%
  % 
  For proof see Section~\ref{proof:covar-of-jac-of-gp}.
\end{lemma}%
% 

\subsubsection{Covariance matrix of Jacobian of GP (Lemma~\ref{lemma:covar-of-jac-of-gp})}
\label{proof:covar-of-jac-of-gp}
\newcommand{\bbfj}{\bar{\bfj}}

Before computing variance, without loss of generality, we consider $J_\bfx f_*(\bfx_*)$
with zero mean.
We write the covariance matrix for $\bfj_* := \vect(J_{\bfx_*} f_*(\bfx_*))$,
% E[fᵢ/x₂, f₃/x₄]
\newcommand{\Epf}[4]{\E\left[\frac{\p f_{#1,*}}{\p x_{#2,*}} \frac{\p f_{#3,*}}{\p x_{#4,*}}\right]}
% E[f/x₁, f/x₂]
\newcommand{\Epbf}[2]{\E\left[\frac{\p \bff_{*}}{\p x_{#1,*}} \frac{\p \bff^\top_{*}}{\p x_{#2,*}}\right]}
%
\begin{align}
  \Cov(\bfj_*, \bfj_*) &:= \E[\bfj_*\bfj_*^\top]
  \\
  \E[\bfj_*\bfj_*^\top] &= \begin{bmatrix}
    \Epbf{1}{1} & \dots & \Epbf{1}{n}
    \\ \vdots & & \vdots \\
    \Epbf{n}{1} & \dots & \Epbf{n}{n}
  \end{bmatrix}
  \\
  \text{where } \Epbf{i}{j} &= \begin{bmatrix}
    \Epf{1}{i}{1}{j} & \dots & \Epf{1}{i}{l}{j}
    \\ \vdots & & \vdots \\
    \Epf{l}{i}{1}{j} & \dots & \Epf{l}{i}{l}{j}
  \end{bmatrix},
\end{align}
%
and we have abbreviated $\bff_* = f_*(\bfx_*)$.

% E[fᵢ/x, fⱼ/x]
\newcommand{\Epfbx}[2]{\E\left[\frac{\p f_{#1,*}}{\p \bfx_{*}} \frac{\p f_{#2,*}}{\p \bfx'_{*}}^\top\right]}
Let us compute the value of $\Epfbx{i}{j}$,

%
\newcommand{\dbfx}{\delta\bfx}
\begin{align}
  \Epfbx{i}{j} &= \lim_{\dbfx,\dbfx' \to 0}\E\left[
  \frac{f_{i,*}(\bfx_* + \dbfx) - f_{i,*}(\bfx_*)}{\dbfx}
  \frac{f_{j,*}(\bfx'_* + \dbfx') - f_{j,*}(\bfx'_*)}{\dbfx'}
  \right]
  \\
               &= \lim_{\dbfx,\dbfx' \to 0}
                 \E\left[\frac{f_{i,*}(\bfx_* + \dbfx)f_{j,*}(\bfx'_* + \dbfx')}{\dbfx \dbfx'}\right]
                 + \E\left[\frac{f_{i,*}(\bfx_*)f_{j,*}(\bfx'_*)}{\dbfx \dbfx'}\right]
  \nonumber\\
               &- \E\left[\frac{f_{i,*}(\bfx_* + \dbfx)f_{j,*}(\bfx'_*)}{\dbfx \dbfx'}\right]
                 - \E\left[\frac{f_{i,*}(\bfx_* )f_{j,*}(\bfx'_* + \dbfx'_*)}{\dbfx \dbfx'}\right]
\end{align}
Note that from Lemma~\ref{thm:multi-variate-gp}, $\E[f_i(\bfx)f_j(\bfx')] =
(k(\bfx, \bfx') - k(\bfx, \bfX)K(\bfX, \bfX)^{-1}k(\bfX, \bfx')) K^f_{i,j}$.
\newcommand{\bfkxd}{\bfk_{\bfx_* + \dbfx}}
\newcommand{\bfkxpd}{\bfk_{\bfx'_* + \dbfx'}}
\begin{align}
  \Epfbx{i}{j}
               &= \lim_{\dbfx,\dbfx' \to 0}
                 \frac{k(\bfx_* + \dbfx, \bfx'_* + \dbfx')
                 - \bfkxd^\top\bfKX\bfkxpd}{\dbfx \dbfx'}K^f_{i,j}
                 \nonumber \\
               & \quad + \frac{k(\bfx_*, \bfx'_*) - \bfkx^\top\bfKX\bfkxp}{\dbfx \dbfx'}K^f_{i,j}
                 - \frac{k(\bfx_* + \dbfx,\bfx'_*)-\bfkxd^\top \bfKX\bfkxp}{\dbfx \dbfx'}K^f_{i,j}
                 \nonumber \\
               & \quad - \frac{k(\bfx_*, \bfx'_* + \dbfx'_*)-\bfkx^\top \bfKX\bfkxpd}{\dbfx \dbfx'}K^f_{i,j}
    %
  \\
  % Arrange terms to look like derivatives
               &= K^f_{i,j}\lim_{\dbfx,\dbfx' \to 0}
                 \frac{1}{\dbfx}\frac{k(\bfx_* + \dbfx, \bfx'_* + \dbfx') - k(\bfx_* + \dbfx,\bfx'_*)}{\dbfx'}
                 \nonumber\\
               & \quad - \frac{1}{\dbfx}\frac{k(\bfx_*, \bfx'_* + \dbfx'_*) - k(\bfx_*, \bfx'_*)}{\dbfx'}
                 - \left(\frac{\bfkxd^\top\bfKX }{\dbfx}\frac{\bfkxpd -  \bfkxp}{\dbfx'} \right)
                 \nonumber \\
                 &\quad+  \left(\frac{\bfkx^\top\bfKX}{\dbfx}\frac{\bfkxpd - \bfkxp}{\dbfx'} \right)
                 % 
  \\
  % Replace with derivatives
               &= K^f_{i,j}\lim_{\dbfx \to 0}
                 \frac{1}{\dbfx}\frac{\p k(\bfx_* + \dbfx, \bfx'_*)}{\p \bfx}
                 - \frac{1}{\dbfx}\frac{\p k(\bfx_*, \bfx'_*)}{\p \bfx}
                 \nonumber \\
               & \quad- \left(\frac{\bfkxd - \bfkx}{\dbfx} \right)^\top \bfKX \frac{\p \bfkxp}{\p \bfx}
  \\
  % Final result
               &= \left( \frac{\p^2 k(\bfx_*, \bfx'_*)}{\p \bfx_*^2}
                 - \frac{\p \bfkx^\top}{\p \bfx}\bfKX \frac{\p \bfkxp}{\p \bfx} \right)K^f_{i,j}. 
\end{align}%
% 
The result is a matrix whose $p,q$ is,
%
\begin{align}
  \Epf{i}{p}{j}{q} = \left[\Epfbx{i}{j}\right]_{p,q} =
  \left[ \frac{\p^2 k(\bfx_*, \bfx'_*)}{\p \bfx_*^2}
                 - \frac{\p \bfkx^\top}{\p \bfx}\bfKX \frac{\p \bfkxp}{\p \bfx} \right]_{p,q}K^f_{i,j}
\end{align}%
% 
Now, we can construction $\Epbf{p}{q}$,
%
\begin{align}
\Epbf{p}{q} &= 
  \left[ \frac{\p^2 k(\bfx_*, \bfx'_*)}{\p \bfx_*^2}
                 - \frac{\p \bfkx^\top}{\p \bfx}\bfKX \frac{\p \bfkxp}{\p \bfx} \right]_{p,q}K^f
\end{align}%
% 
Hence, the full covariance matrix becomes,
%
\begin{align}
\Cov(\bfj_*, \bfj_*) &= 
  \left[ \frac{\p^2 k(\bfx_*, \bfx'_*)}{\p \bfx_*^2}
                 - \frac{\p \bfkx^\top}{\p \bfx}\bfKX \frac{\p \bfkxp}{\p \bfx} \right] \otimes K^f
  \\
  &= \left[ H_{xx} k(\bfx_*, \bfx'_*)
    - J_{\bfx_*}^\top \bfkx\bfKX J_{\bfx_*}\bfkxp \right] \otimes K^f
\end{align}%
% 

\hfill $\blacksquare $

==> tex/old/differentiating-gp.tex <==
%\section{Differentiating Random Process} 
%\begin{proof}[Proof of Lemma~\ref{lemma:differentiating-gp}]

\section{Proof of Lemma~\ref{lemma:differentiating-gp}}
\label{proof:differentiating-gp}

Let $q(\bfx)$ be a scalar random process with finite differentiable $\mu(\bfx)$ mean and finite twice differentiable variance $\knl(\bfx, \bfx')$ for all $\bfx \in \calX$. 
Next we compute the mean and variance of random process $\grad_\bfx q(\bfx)$,\NA{The expression for computing the gradient below is only valid for scalars. Also, how do you exchange the expectation and derivative? There are certain conditions for being able to do so.}
%
\newcommand{\dbfy}{\delta \bfy}
\newcommand{\dbfx}{\delta \bfx}
\begin{equation}
\begin{aligned}
\E[\grad_\bfx q(\bfx)] 
&= \lim_{\dbfx \to 0} \frac{1}{\dbfx}\E[ q(\bfx + \dbfx) - q(\bfx)]
  \\
&= \lim_{\dbfx \to 0} \frac{1}{\dbfx}\E[ q(\bfx + \dbfx)] - \E[q(\bfx)]
\\
&= \lim_{\dbfx \to 0} \frac{1}{\dbfx}\bigl(\mu(\bfx + \dbfx) - \mu(\bfx)\bigr)
= \grad_\bfx \mu(\bfx)
\end{aligned}%
\end{equation}
% 

To compute kernel function, consider a random process with zero mean, $ z(\bfx) = q(\bfx) -
\mu(\bfx)$ but same variance as $q$.
We write differentiation as limit of finite differences,\NA{Again, how do you exchange the expectation and derivative? What is $\dbfx$?}
%
\begin{align}
  &\bfK_{\grad q}(\bfx, \bfy) = \knl_{\grad z}(\bfx, \bfy) = \E[\grad z(\bfx) \grad z(\bfy)^\top]
  \\\notag
  &= \lim_{\dbfx,\dbfy \to 0}\E\left[
  \left(\frac{z(\bfx + \dbfx) - z(\bfx)}{\dbfx}\right)
  \left(\frac{z(\bfy + \dbfy) - z(\bfy)}{\dbfy}\right)^\top
  \right],
\end{align}
 where 
\begin{align}& \frac{z(\bfx + \dbfx) - z(\bfx)}{\dbfx} = \begin{bmatrix}
\frac{z(\bfx + \dbfx) - z(\bfx)}{\delta x_1} & \dots & \frac{z(\bfx + \dbfx) - z(\bfx)}{\delta x_n}.
    \end{bmatrix}
\end{align}%
% 
%
Considering only $i,j$th element of the kernel,
%
\newcommand{\dyj}{\delta y_j}
\newcommand{\dxi}{\delta x_i}
\begin{align}
  &[\bfK_{\grad q}(\bfx, \bfy)]_{i,j}
  \notag\\
  &=
    \lim_{\dxi, \dyj \to 0} \E\left[
  \frac{z(\bfx + \dbfx) - z(\bfx)}{\dxi}
  \frac{z(\bfy + \dbfy) - z(\bfy)}{\dyj}
                          \right]
    \notag\\
    &=
    \lim_{\dxi, \dyj \to 0} 
      \frac{1}{\dxi\dyj}\Bigl(\E[z(\bfx + \dbfx)z(\bfy + \dbfy)]
      \notag\\&\qquad
      - \E[z(\bfx)z(\bfy + \dbfy)] 
  - \E[z(\bfx + \dbfx)z(\bfy)]
  \notag\\&\qquad
  + \E[z(\bfx)z(\bfy)] \Bigr)
  \notag\\
  &=
    \lim_{\dxi, \dyj \to 0} 
      \frac{1}{\dxi\dyj}\Bigl(\knl(\bfx + \dbfx, \bfy + \dbfy)
    - \knl(\bfx + \dbfx, \bfy)
  \notag\\&\qquad
      - [\knl(\bfx, \bfy + \dbfy) - \knl(\bfx, \bfy)] \Bigr)
  \notag\\
  &=
  \frac{ \p^2 \knl(\bfx,\bfy) }
  {\p x_i \p y_j }
\end{align}%
% 
Hence, the resultant kernel function is the Hessian of the kernel $\bfK_{\grad q}(\bfx, \bfy) = \calH_{\bfx,
  \bfy}\knl(\bfx, \bfy)$. $\grad q$ can be written as a Vector-variate Gaussian  Process,
%
\begin{align}
\grad q &\sim \GP(\grad \mu, \bfK_{\grad q}) & \text{where } \bfK_{\grad q}(\bfx, \bfx') &= \calH_{\bfx, \bfx'} \knl(\bfx, \bfx')
\end{align}%
% 
We assume another vector-valued Gaussian process $s(\bfy)$ with mean
$\bar{s}(\bfy)$ and known covariance with $q(\bfx)$ as $\cov_{q,s}(\bfx, \bfy)$.
To prove that $ \cov(\grad q(\bfx), s(\bfy)) = \grad_\bfx\cov_{q,s}(\bfx,
\bfy)$, we start with
%
\begin{equation}
\begin{aligned}
  \cov(\grad q, s)
  &= \E[ (\grad q(\bfx) - \grad \mu(\bfx)) (s(\bfy) - \bar{s}(\bfy))^\top ]
    \\
    &= \E[\grad q(\bfx) s(\bfy)^\top ] -  \grad \mu(\bfx) \bar{s}(\bfy)^\top
    \label{eq:diff-gp-cov-with-mean}
\end{aligned}
\end{equation}
%
Expanding the first term,
%
\begin{align}
  \E[&\grad q(\bfx) s(\bfy)^\top ]
  = \lim_{\dbfx\to 0}\E\left[
  \frac{q(\bfx + \dbfx) - q(\bfx)}{\dbfx} s(\bfy)^\top
  \right],
  \notag\\
  &= \lim_{\dbfx\to 0}
  \frac{\E[q(\bfx + \dbfx)s(\bfy)^\top] - \E[q(\bfx) s(\bfy)^\top]}{\dbfx}
  \notag\\
  &=
    \lim_{\dbfx\to 0} \frac{1}{\dbfx}\big(\cov_{q,s}(\bfx + \dbfx, \bfy) +
\mu(\bfx + \dbfx)\bar{s}(\bfy)^\top 
    \notag\\&\qquad
- \cov_{q,s}(\bfx, \bfy)-
    \mu(\bfx)\bar{s}(\bfy)^\top \big)
  \notag\\
  &=
    \grad_\bfx \cov_{q,s}(\bfx, \bfy) + \grad_\bfx \mu(\bfx)\bar{s}(\bfy)^\top
    \label{eq:diff-gp-cov-no-mean}
\end{align}%
% 
From \eqref{eq:diff-gp-cov-with-mean} and \eqref{eq:diff-gp-cov-no-mean}, we get
$\cov(\grad q(\bfx), s(\bfy)) = \grad_\bfx \cov_{q,s}(\bfx, \bfy)$.

To prove that $\cov(\grad q(\bfx), q(\bfx)) = \grad_\bfx \knl(\bfx, \bfx')$,
substitute $s = q$. \qed





==> tex/old/differentiating-lie.tex <==
\subsubsection{Differentiating Gradient of Lie~\eqref{eq:mean-var-grad-lie-grad-h-f-expanded}}
\label{proof:differentiating-lie}

\begin{align}
    \bbH(\bfx, \bfy) \triangleq \calH_{\bfx, \bfy} \left[ \knl(\bfx, \bfy)\grad h(\bfx)^\top K^f \grad h(\bfy) \right]
\end{align}

\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\pdd}[3]{\frac{\partial #1}{\partial #2 \partial #3}}
\begin{align}
  &\left[ \bbH(\bfx, \bfy) \right]_{i,j}
    = \pdd{}{x_i}{y_j}  \left[ 
    \knl(\bfx, \bfy)\grad h(\bfx)^\top K^f \grad h(\bfy) 
    \right]
    \\
    &= \pd{}{x_i} \left[ 
    \pd{\knl(\bfx, \bfy)}{y_j} \grad h(\bfx)^\top K^f \grad h(\bfy) 
      \right.\nonumber\\&\qquad\left.
    + \knl(\bfx, \bfy)\grad h(\bfx)^\top K^f \pd{\grad h(\bfy)}{y_j}
    \right]
    \\
    &= 
    \pdd{\knl(\bfx, \bfy)}{x_i}{y_j} \grad h(\bfx)^\top K^f \grad h(\bfy) 
\nonumber\\&\qquad
    + \pd{\knl(\bfx, \bfy)}{y_j} \pd{\grad h(\bfx)^\top}{x_i} K^f \grad h(\bfy) 
\nonumber\\&\qquad
    + \pd{\knl(\bfx, \bfy)}{x_i}\grad h(\bfx)^\top K^f \pd{\grad h(\bfy)}{y_j}
\nonumber\\&\qquad
    + \knl(\bfx, \bfy)\pd{\grad h(\bfx)^\top}{x_i} K^f \pd{\grad h(\bfy)}{y_j}
\end{align}

Considering matrix forms of each of the terms in above equation, 
\begin{align}
[\calH_{\bfx, \bfy}&\knl(\bfx, \bfy)]_{i,j} \grad h(\bfx)^\top K^f \grad h(\bfy) ]_{i,j}
  \nonumber\\
&= 
    \pdd{\knl(\bfx, \bfy)}{x_i}{y_j} \grad h(\bfx)^\top K^f \grad h(\bfy) 
    \\
    [ \grad &h(\bfy)K^{f\top}  \calH_{xx} h(\bfx) \grad_\bfy \knl(\bfx, \bfy)^\top]_{i,j} 
              \nonumber\\
    &=  \pd{\knl(\bfx, \bfy)}{y_j} \pd{\grad h(\bfx)^\top}{x_i} K^f \grad h(\bfy) 
    \\
    [\grad_\bfx& \knl(\bfx, \bfy) \grad h(\bfx)^\top K^f \calH_{yy} h(\bfy)]_{i,j} 
              \nonumber\\
    &= \pd{\knl(\bfx, \bfy)}{x_i}\grad h(\bfx)^\top K^f \pd{\grad h(\bfy)}{y_j}
    \\
    [\knl(\bfx, \bfy)& \calH_{xx} h(\bfx) K^f \calH_{yy} h(\bfy)]_{i,j}
              \nonumber\\
    &= \knl(\bfx, \bfy)\pd{\grad h(\bfx)^\top}{x_i} K^f \pd{\grad h(\bfy)}{y_j}
\end{align}

Hence,
\begin{align}
\bbH(\bfx, \bfy) 
&= \calH_{\bfx, \bfy}\knl(\bfx, \bfy) \grad h(\bfx)^\top K^f \grad h(\bfy)
                    \nonumber\\&\qquad
+ \grad h(\bfy)K^{f\top}  \calH_{xx} h(\bfx) \grad_\bfy \knl(\bfx, \bfy)^\top
  \nonumber\\&\qquad
+ \grad_\bfx \knl(\bfx, \bfy) \grad h(\bfx)^\top K^f \calH_{yy} h(\bfy)
  \nonumber\\&\qquad
+ \knl(\bfx, \bfy) \calH_{xx} h(\bfx) K^f \calH_{yy} h(\bfy)
\end{align}

==> tex/old/mean-of-jac-of-gp.tex <==
%
\begin{lemma}[Mean of Jacobian of Gaussian Process]
  \label{thm:mean-of-jac-of-gp}
Under assumptions of Lemma~\ref{thm:multi-variate-gp}, the Jacobian of
posterior GP, $J_{\bfx_*} f_*(\bfx) \in \R^{l \times n}$, is also Gaussian.
The mean of the vectorized $\bfj_* := \vect(J_{\bfx_*} f_*(\bfx_*)) \in \R^{ln}$ is given by,
% 
  \begin{align}
    \bar{\bfj}_* := \E[\vect(J_{\bfx_*} f_*(\bfx_*))] &= \left[[J_{\bfx_*}^\top \bfkx \bfKX] \otimes I_{l \times l}\right] \bfY.
  \end{align}%
  % 
  For scalar-valued GP put $l=1$, 
% 
  \begin{align}
    \bar{\bfj}_* := \E[\grad_\bfx f_*(\bfx_*)] &= J_{\bfx_*}^\top \bfkx \bfKX \bfY.
  \end{align}%
  % 
  For proof see Section~\ref{proof:mean-of-jac-of-gp}.
\end{lemma}%
% 

\subsubsection{Mean of Jacobian of Gaussian process(Lemma~\ref{thm:mean-of-jac-of-gp})}
\label{proof:mean-of-jac-of-gp}
Since jacobian is a linear operator, we can compute the mean by swapping
expectation and jacobian,
%
\begin{align}
  \E[\vect(J_{\bfx_*} f_*(\bfx_*))] &= \vect(J_{\bfx_*} \E[f_*(\bfx)]) =
                          \vect\left( J_{\bfx_*} \left\{ \left[[k(\bfx_*, \bfX)K(\bfX, \bfX)^{-1}] \otimes I_{l \times l}\right] \bfY \right\} \right)
\end{align}


\begin{align}
  \E[\vect(J_{\bfx_*} f_*(\bfx_*))] =
  \vect\Bigl( J_{\bfx_*}& \left\{ \left[[k(\bfx_*, \bfX)K(\bfX, \bfX)^{-1}] \otimes I_{l \times l}\right] \bfY \right\} \Bigr)
  \\
                        &= \begin{bmatrix}
                          \frac{\p }{\p x_{1,*}} \left[[k(\bfx_*, \bfX)K(\bfX, \bfX)^{-1}] \otimes I_{l \times l}\right] \bfY
                          \\ \vdots \\
                          \frac{\p }{\p x_{n,*}} \left[[k(\bfx_*, \bfX)K(\bfX, \bfX)^{-1}] \otimes I_{l \times l}\right] \bfY
                        \end{bmatrix}
  \\
                        &= \begin{bmatrix}
                          \left[[\frac{\p }{\p x_{1,*}} k(\bfx_*, \bfX)K(\bfX, \bfX)^{-1}] \otimes I_{l \times l}\right] \bfY
                          \\ \vdots \\
                          \left[[\frac{\p }{\p x_{n,*}} k(\bfx_*, \bfX)K(\bfX, \bfX)^{-1}] \otimes I_{l \times l}\right] \bfY
                        \end{bmatrix}
  \\
                        &= \begin{bmatrix}
                          [\frac{\p }{\p x_{1,*}} k(\bfx_*, \bfX)K(\bfX, \bfX)^{-1}] \otimes I_{l \times l}
                          \\ \vdots \\
                          [\frac{\p }{\p x_{n,*}} k(\bfx_*, \bfX)K(\bfX, \bfX)^{-1}] \otimes I_{l \times l}
                          \end{bmatrix} \bfY
  \label{eq:mean-jac-pre-vcat}
\end{align}

Consider the Kronecker product of vertical concatenation of matrices,
%
\begin{align}
  \begin{bmatrix} A \otimes B \\ C \otimes B\end{bmatrix}
  = \begin{bmatrix}
    A_{11}B & \dots & A_{1n} B
    \\ \vdots && \vdots \\
    A_{n1}B & \dots & A_{nn} B \\
    C_{11}B & \dots & C_{1n} B
    \\ \vdots && \vdots \\
    C_{n1}B & \dots & C_{nn} B \\
  \end{bmatrix}
  = \begin{bmatrix} A \\ C \end{bmatrix} \otimes B
  \label{eq:prop-kronecker-vcat}
\end{align}%
% 

Apply property \eqref{eq:prop-kronecker-vcat} to \eqref{eq:mean-jac-pre-vcat},
%
\begin{align}
  \E[\vect(J_{\bfx_*} f_*(\bfx_*))] &= \begin{bmatrix}
    \left[ \begin{bmatrix}
      \frac{\p }{\p x_{1,*}} k(\bfx_*, \bfX)
      \\ \vdots \\
      \frac{\p }{\p x_{n,*}} k(\bfx_*, \bfX)
    \end{bmatrix}
    K(\bfX, \bfX)^{-1} \right] \otimes I_{l \times l}
    \end{bmatrix}\bfY
\end{align}%
% 

\begin{align}
  \E[\vect(J_{\bfx_*} f_*(\bfx_*))]
  &= \left[[J_{\bfx_*}^\top k(\bfx_*, \bfX) K(\bfX, \bfX)^{-1}] \otimes I_{l \times l}\right] \bfY
  \\
  &= \left[[J_{\bfx_*}^\top \bfkx \bfKX] \otimes I_{l \times l}\right] \bfY.
\end{align}
\hfill $\blacksquare $

==> tex/old/moreonECBF.tex <==
If $\bfk_\alpha$ satisfies the properties stated in in the next theorem, any control policy $\bfu = \pi(\bfx)$ that ensures $\mbox{CBC}^{(r)} \ge 0$, renders the dynamics~\eqref{eq:system_dyanmics} safe with respect to set $\mathcal{C}$.
\begin{theorem}[Designing $\bfk_\alpha$~\cite{nguyen2016exponential,cbf}]
  Function $h(\bfx)$ is Exponential CBF if $\bfk_\alpha$ is chosen with following
  conditions.
  \begin{enumerate}
    \item $\mathcal{F} - \mathcal{G}\bfk_\alpha$ is Hurwitz and total negative
      (resulting in negative real poles).
    \item The eigenvalues $\lambda_i$ of the system \eqref{eq:traverse-system}
      satisfy
      $\lambda_i (\mathcal{F} - \mathcal{G}\bfk_\alpha) \ge
      -\frac{\dot{\nu}_{i-1}(\bfx_0)}{\nu_{i-1}(\bfx_0)}$, where $\nu_i(\bfx)$
      is recursively defined as $\nu_0(\bfx) := h(\bfx)$, $\nu_i(\bfx) := \dot{\nu}_{i-1} +
      p_i\nu_{i-1}(\bfx)$, with $\{p_i\}_{i=1}^r$  as
    the $r$ roots of the characteristic polynomial of the matrix
    $\mathcal{F} - \mathcal{G}\bfk_\alpha$.
  \end{enumerate}
\end{theorem}

For relative degree one systems $\bfk_\alpha^\top \eta(\bfx)$ reduces to $\alpha h(\bfx)$ with $\alpha>0$. Thus, $CBC^{(1)}$, the safety condition based on ECBF, is equivalent to CBC in Def.~\ref{def:cbf} when  $\alpha$, the extended class $K_\infty$ function, is linear.

==> tex/old/multi-variate-gp.tex <==
\subsubsection{Multi-variate Gaussian Process (Eq~\eqref{eq:mvg-posterior})}
\label{proof:multi-variate-gp}

Consider $f(\bfx_i) = \vect{\dynAff(\bfx_i)}$ and $K^f = \bfB \otimes \bfA \in
\R^l$, where $l = mn$.
Then $f(\bfx, \bfx') \sim \GP(0, k(\bfx, \bfx')K^f)$.

\newcommand{\bfkx}{\bfk_{\bfx_*}}
\newcommand{\bfKX}{\bfK^{-1}_\bfX}
\newcommand{\bfkxp}{\bfk_{\bfx'_*}}

The joint distribution between test data and train data is Gaussian,
%
\begin{align}
  \begin{bmatrix}
    f(\bfx_1)
    \\ \vdots \\
    f(\bfx_d)
    \\
    f(\bfx_*)
  \end{bmatrix}
  &\sim
  \N\left(
  % mean
  \begin{bmatrix}
    \mathbf{0}_{l}
    \\ \vdots \\
    \mathbf{0}_{l}
    \\
    \mathbf{0}_{l}
  \end{bmatrix},
  % covar
  \begin{bmatrix}
    k(\bfx_1, \bfx_1)K^f & \dots & k(\bfx_1, \bfx_d)K^f & k(\bfx_1, \bfx_*) K^f
    \\ \vdots & & \vdots & \vdots \\
    k(\bfx_d, \bfx_1)K^f & \dots & k(\bfx_d, \bfx_d)K^f & k(\bfx_d, \bfx_*) K^f
    \\
    k(\bfx_*, \bfx_1)K^f & \dots & k(\bfx_*, \bfx_d)K^f & k(\bfx_*, \bfx_*) K^f
  \end{bmatrix}
                                                          \right)
  \\
  \begin{bmatrix}
    \bfY
    \\
    f(\bfx_*)
  \end{bmatrix}
  &\sim
  \N\left(
  % mean
  \begin{bmatrix}
    \mathbf{0}_{dl}
    \\
    \mathbf{0}_{l}
  \end{bmatrix},
  % covar
  \begin{bmatrix}
    K(\bfX, \bfX) \otimes K^f & k(\bfX, \bfx_*) \otimes K^f
    \\
    k(\bfx_*, \bfX) \otimes K^f & k(\bfx_*, \bfx_*) \otimes K^f
  \end{bmatrix}
                                                          \right),
\end{align}%
% 
where $k(\bfx_*, \bfX) := [k(\bfx_*, \bfx_1), \dots, k(\bfx_*, \bfx_d)]^\top =:
k(\bfX, \bfx_*)^\top$, and $K(\bfX, \bfX) := [k(\bfx_i, \bfx_j)]_{i=1,j=1}^{n,n}$.

The posterior of GP on a test point $\bfx_*$ is given by,
%
\begin{align}
  f_*(\bfx_*) := f(\bfx_*) | \bfX, \bfY &\sim \N\Bigl(
    % mean
  (k(\bfx_*, \bfX) \otimes K^f) (K(\bfX, \bfX)  \otimes K^f)^{-1} \bfY,
  % covar
  \\&
  (k(\bfx_*, \bfx_*) \otimes K^f) -
  (k(\bfx_*, \bfX) \otimes K^f) (K(\bfX, \bfX)  \otimes K^f)^{-1} (k(\bfX, \bfx_*) \otimes K^f)
  \Bigr).
\end{align}%
% 

By using properties of Kronecker product
$(A \otimes B)(C \otimes D) = AC \otimes BD$,
$(A \otimes B)^{-1} = A^{-1} \otimes B^{-1}$,
$(A \otimes C + B \otimes C) = (A + B) \otimes C$, we get
%
%
\begin{align}
  f_*(\bfx_*)
  & \sim \N\Bigl(
  % mean
  \left[[k(\bfx_*, \bfX)K(\bfX, \bfX)^{-1}] \otimes I_{l}\right] \bfY,
  % covar \\&
  [k(\bfx_*, \bfx_*) -k(\bfx_*, \bfX) K(\bfX, \bfX)^{-1} k(\bfX, \bfx_*)] K^f
  \Bigr)
  \\
  &=
    \N\Bigl(
    % mean
  \left[[\bfkx \bfKX] \otimes I_{l}\right] \bfY,
  % covar \\&
  [k(\bfx_*, \bfx_*) -\bfkx^\top \bfKX \bfkx] K^f
  \Bigr),
\end{align}%
% 
where $I_{l} \in \R^{l}$ is identity matrix.

Substitute $K^f = \bfB \otimes \bfA$ and $I_l = I_n \otimes I_m$.
\hfill  $ \blacksquare $

==> tex/old/old-mean-variance-of-cbc-2.tex <==
%\documentclass[../main.tex]{subfiles}
%\begin{document}
\subsubsection{Mean and Variance of $\CBCtwo$~\ref{sec:exp-cbf-rel-deg-2}}
\label{proof:mean-var-of-cbc}
\newcommand{\mean}[1]{\bbE[{#1}]}
%

%For ease of notation, define $\tdbff(\bfx; \bfu) := f_k(\bfx)+ g_k(\bfx)\ctrl :=
%\dynAff_k(\bfx)\ctrlaff$.
The mean, variances and covariances
of different components are given by (using~Lemma~\ref{lemma:product-mvg}),
%
\begin{align}
  \text{Let } \bfB_k(\bfx, \bfx') &:= \begin{bmatrix}
    b_{f_k}(\bfx, \bfx') & \bfb_k(\bfx, \bfx')^\top
    \\
    \bfb_k(\bfx, \bfx') & \bfB_{g_k}(\bfx, \bfx')
    \end{bmatrix}
  \\
  \mutdf(\bfx) &:=  \mDynAffs(\bfx) [1, \bfzero_m]^\top,
  \\
  \Var(f_k(\bfx)) &= [1, \bfzero_m] \bfBs(\bfx, \bfx') [1, \bfzero_m]^\top\bfA
  \\
  &= b_{f_k}(\bfx, \bfx') \bfA
                                        \label{eq:mvg-posterior-f}
  \\
  \mutdgu(\bfx) &:= \mDynAffs(\bfx) [0, \bfone^\top]^\top,
  \\
  \Var(\vect(g_k(\bfx))) &= [0, \bfone^\top] \bfBs(\bfx, \bfx') [0, \bfone^\top]^\top \otimes \bfA
  \\
                         &= \ktdgu(\bfx, \bfx') \otimes \bfA
  \\
  \Var(\dynAff(\bfx)\ctrlaff) &= \ctrlaff^\top \bfBs(\bfx, \bfx') \ctrlaff \bfA
                                                    \label{eq:mvg-posterior-bfu}
  \\
               \cov(f_k(\bfx), \vect(\dynAff_k(\bfx')))
  &= [1, \bfzero_m] \bfBs(\bfx, \bfx') \otimes \bfA.
  \\
  &= \bfb_k(\bfx, \bfx') \otimes \bfA
\end{align}%
% 
Note that all the variances are expressed as a scalar kernel function times $\bfA$.



% We derive the mean and variance and bounds over $\CBCtwo$.
% Then condition
% $\LieTwo h(\bfx)$ can be written as a quadratic form in the random
% vectors $\bfz(\bfx) := [\grad \LieOne h(\bfx)^\top, \vect(\dynAff(\bfx)), \LieOne  h(\bfx)]^\top$ ,
% %
% \begin{align}
%   [\LieTwoF(\bfx), \LieTwoG(\bfx)]
%   := \grad \LieOne h(\bfx)^\top \dynAff_k(\bfx)
%    = \bfz(\bfx)^\top
%   \underbrace{\begin{bmatrix}
%     0 & \frac{I_n}{2} &  0 \\
%     \frac{I_n}{2} & 0 &  0 \\
%     0 & 0 & 0
%   \end{bmatrix}}_{=: \Lambda }
%             \bfz(\bfx)
%   \label{eq:cbc-quadratic-form}
% \end{align}%
% % 
% 
% The challenge is to compute the mean and variance of vector-variate Gaussian process $\bfz(\bfx)$.

We will compute the mean and variance of each of the term one by one.
We compute it in three main steps, computation of mean and variance of (1) $\LieOne h(\bfx)$, (2) $\grad \LieOne h(\bfx)$ and (3) $ \dynAff(\bfx)^\top \grad \LieOne h(\bfx)$.

\paragraph{Step 1: Mean and variance of $\LieOne h(\bfx)$}
We start by observing that $\LieOne h(\bfx) = \grad h(\bfx)^\top f_k(\bfx) $ is a
scalar value Gaussian process because $\grad h(\bfx)$ is deterministic,
%
%
\begin{equation}\begin{split}%
  \LieOne h &\sim \GP\left(\mean{\LieOne h} , \knl_{\LieOne h} \right)
  \\
  \text{where } \mean{\LieOne h} (\bfx) &= \grad h(\bfx)^\top \mutdf(\bfx)
  \\
  \knl_{\LieOne h}(\bfx, \bfx') &= b_{f_k}(\bfx, \bfx') \grad h(\bfx)^\top \bfA \grad h(\bfx').
  \\
  \cov( \LieOne h(\bfx), &\vect(\dynAff_k(\bfx'))) 
  \\
  &= \grad^\top h(\bfx) \cov(f_k(\bfx), \vect(\dynAff_k(\bfx))) 
  \nonumber \\
  &=  \grad h(\bfx)^\top (\bfb_k(\bfx, \bfx')^\top \otimes \bfA)
  \\
  &=  (1 \otimes \grad h(\bfx)^\top) (\bfb_k(\bfx, \bfx')^\top \otimes \bfA)
  \\
  &=  \bfb_k(\bfx, \bfx')^\top \otimes \grad h(\bfx)^\top \bfA
  \\
  &=  \bfb_k(\bfx, \bfx')^\top \otimes \grad h(\bfx)^\top \bfA \in \R^{1 \times (m+1)n}
  \\
  \cov( \LieOne h(\bfx), &\dynAff_k(\bfx')\ctrlaff) 
  = \grad h(\bfx)^\top \bfA (\bfb_k(\bfx, \bfx')^\top \ctrlaff)
  \label{eq:mean-var-lie-grad-h-f}
\end{split}\end{equation}%
% 

%
\begin{lemma}[Gradient of a Gaussian Process]
  \label{lemma:differentiating-gp-copy}
  Let $q$ be a scalar valued Gaussian Process with mean function
$\mu : \R^n \to \R$ and kernel function $\knl : \R^n \to \R$, then $\grad q$ is a vector-valued Gaussian
Process,
%
\begin{align}
  \grad q &\sim \GP(\grad \mu, K_{\grad q}) \\
  \text{where }&  K_{\grad q}(\bfx, \bfx') = \calH_{\bfx, \bfx'} \knl(\bfx, \bfx')
                                                                                     \\
&\cov(\grad q(\bfx), q(\bfx')) = \grad_{\bfx} \knl(\bfx, \bfx').
\end{align}

If $s$ is another random process whose finite covariance with $q$ is known to be
$\cov_{q,s}(\bfx, \bfx')$, then
\begin{align}
\cov(\grad q(\bfx), s(\bfx')) = \grad_\bfx \cov_{q,s}(\bfx, \bfx').
\end{align}%
For proof see Section~\ref{proof:differentiating-gp}. Note that the expressions for mean, variance and covariance are valid for any random process, even if not Gaussian.
\end{lemma}%
% 

Using Lemma~\ref{lemma:differentiating-gp} $\grad \LieOne h(\bfx)$ is a
vector-variate Gaussian Process,
%
\begin{equation}\begin{split}%
  \grad \LieOne h &\sim \GP(\mean{\grad \LieOne h}, K_{\grad \LieOne h})
  \\
  \text{ where }&
  \mean{\grad \LieOne h}(\bfx) = \grad_\bfx \mean{\LieOne h} (\bfx)
  \\
  &K_{\grad \LieOne h}(\bfx, \bfx') = \calH_{\bfx,\bfx'} [  \knl_{\LieOne h}(\bfx, \bfx') ]
    \\
    & \cov(\grad \LieOne h(\bfx), \LieOne h(\bfx)) = \grad_\bfx  \knl_{\LieOne h}(\bfx, \bfx')
    \\
    & \cov(\grad \LieOne h(\bfx), \vect(\dynAff_k(\bfx'))) 
    \\
    &\qquad \qquad= \grad_\bfx  \cov(\LieOne h(\bfx), \vect(\dynAff_k(\bfx')))
\label{eq:mean-var-grad-lie-grad-h-f}
\end{split}\end{equation}%
%

The above derivatives can be expanded as,
%
\begin{multline}
  \mean{\grad \LieOne h}(\bfx) = \calH_{\bfx,\bfx}[h(\bfx)] \mutdf(\bfx) + J^\top_\bfx [\mutdf(\bfx)] \grad h(\bfx)
\end{multline}
\begin{multline}
% Variance
  K_{\grad \LieOne h}(\bfx, \bfx')
= \calH_{\bfx, \bfx'}[b_{f_k}(\bfx, \bfx')] \grad h(\bfx)^\top \bfA \grad h(\bfx')
\\
+ \grad h(\bfx')\bfA^{\top}  \calH_{xx} [h(\bfx)] \grad_{\bfx'} [b_{f_k}(\bfx, \bfx')]^\top
\\
+ \grad_\bfx [b_{f_k}(\bfx, \bfx')] \grad h(\bfx)^\top \bfA \calH_{xx} [h(\bfx')]
\\
+ b_{f_k}(\bfx, \bfx') \calH_{xx} h(\bfx) \bfA \calH_{xx} [h(\bfx')]
    \; \text{(See ~\ref{proof:differentiating-lie})}
\end{multline}
\begin{multline}
% Covariance with respect to parent
  \cov(\grad \LieOne h(\bfx), \LieOne h(\bfx'))
  \\
  = \grad_\bfx b_{f_k}(\bfx, \bfx') \grad h(\bfx)^\top \bfA \grad h(\bfx') 
  \\
  + b_{f_k}(\bfx, \bfx') \grad h(\bfx') \bfA^\top \calH_{xx}[h(\bfx)]
\end{multline}
\begin{multline}
% Covariance
  \cov(\grad \LieOne h(\bfx)), \vect(\dynAff(\bfx')))
  \\
  = (\calJ_\bfx^\top \bfb_k(\bfx,\bfx') \otimes \grad h(\bfx)^\top \bfA) 
  \\
    +  (\bfb_k(\bfx,\bfx')^\top \otimes H^\top_{xx}[h(\bfx)]\bfA )
    \in \R^{n \times (m+1)n}
\label{eq:mean-var-grad-lie-grad-h-f-expanded}
\end{multline}%



%
Now we are equipped to compute mean and variance of $\dynAff(\bfx)^\top \grad_\bfx \LieOne  h(\bfx) $:
%
\begin{multline}
  \E[\dynAff(\bfx)^\top \grad \LieOne  h(\bfx) ]
  = 
  \bfM_k(\bfx)^\top \E[\grad \LieOne h(\bfx)]
  \\
  + 
  \begin{bmatrix}
  \tr(\cov( \grad \LieOne h(\bfx), f_k(\bfx) ))
  \\
  \tr(\cov( \grad \LieOne h(\bfx), g_k(\bfx)_1 ))
  \\
  \vdots
  \\
  \tr(\cov( \grad \LieOne h(\bfx), g_k(\bfx)_n ))
  \end{bmatrix}
\end{multline}

We know from  \eqref{eq:mean-var-grad-lie-grad-h-f-expanded}, $\cov(\grad \LieOne h(\bfx), \vect(\dynAff_k(\bfx)))$,
\begin{multline}
    \cov(\grad \LieOne h(\bfx), \vect(\dynAff_k(\bfx))) 
    \\
    = \calJ_\bfx[ \bfb_k(\bfx, \bfx') ]^\top \otimes \grad_\bfx h(\bfx)^\top A
    \\
    + \bfb_k(\bfx, \bfx')^\top \otimes \calH_{\bfx, \bfx} h(\bfx)^\top A.
\end{multline}
Since $\vect(\dynAff_k(\bfx)) = [f_k(\bfx)^\top, g_k(\bfx)_1^\top, \dots, g_k(\bfx)_m^\top]^\top$, 
we can compute the covariance for each column,
\begin{multline}
    \cov(\grad \LieOne h(\bfx), \dynAff_k(\bfx)_{:, i})
    \\
    = [\calJ_\bfx[ \bfb_k(\bfx, \bfx') ]_{i, :}]^\top \otimes \grad_\bfx h(\bfx)^\top A
    \\
    + \bfb_k(\bfx, \bfx')_{i}^\top \otimes \calH_{\bfx, \bfx} h(\bfx)^\top A.
\end{multline}
Note that the first term is simply the outer product of a row vector and column vector and the second term is scalar times a matrix.
Taking trace of each term we get,
\begin{multline}
    \tr(\cov(\grad \LieOne h(\bfx), \dynAff_k(\bfx)_{:, i}))
    \\
    = [\calJ_\bfx[ \bfb_k(\bfx, \bfx') ]_{i, :}]^\top A \grad_\bfx h(\bfx)
    \\
    + \bfb_k(\bfx, \bfx')_{i}^\top \tr(\calH_{\bfx, \bfx} h(\bfx)^\top A)
\end{multline}
We put the terms in \eqref{eq:lie-2-mean-app}, to get,
\begin{multline}
  \E[\dynAff(\bfx)^\top \grad \LieOne  h(\bfx) ]
  \\
  = 
  \bfM_k(\bfx)^\top \E[\grad \LieOne h(\bfx)]
  \\
  + 
  \calJ_\bfx[ \bfb_k(\bfx, \bfx') ]^\top A \grad_\bfx h(\bfx)
    + \bfb_k(\bfx, \bfx') \tr(\calH_{\bfx, \bfx} h(\bfx)^\top A)
\end{multline}
\begin{multline}
  \E[\dynAff(\bfx)^\top \grad \LieOne  h(\bfx) ]
  \\
  = 
    \bfM_k(\bfx)^\top
  \bigl(
      \calH_{\bfx,\bfx}[h(\bfx)] \mutdf(\bfx) + J^\top_\bfx[ \mutdf(\bfx)] \grad h(\bfx)
    \bigr)
    \\
  + \calJ_\bfx[ \bfb_k(\bfx, \bfx') ]^\top A \grad_\bfx h(\bfx)
    + \bfb_k(\bfx, \bfx') \tr(\calH_{\bfx, \bfx} h(\bfx)^\top A)
  \label{eq:lie-2-mean-app}
\end{multline}

We do not know the covariance of quadratic forms with each other, so it is hard to 
compute the variance of $\dynAff_k(\bfx)^\top \grad \LieOne h(\bfx)$, but 
we eventually only need the variance of $ \ctrlaff^\top \dynAff_k(\bfx)^\top \grad \LieOne h(\bfx)$
\begin{multline}
  \Var[\ctrlaff^\top \dynAff_k(\bfx)^\top \grad \LieOne  h(\bfx)]
  \\
  = 
  2\tr(\cov(\grad \LieOne h(\bfx), \dynAff_k(\bfx)\ctrlaff)))^2
    \\
    + \E[\grad \LieOne h(\bfx)]^\top 
    \cov(\grad \LieOne h(\bfx), \dynAff_k(\bfx)\ctrlaff )
    \bfM_k(\bfx) \ctrlaff 
    \\
    +  \E[\grad \LieOne h(\bfx)]^\top (\ctrlaff^\top \bfB \ctrlaff \bfA) \E[\grad \LieOne h(\bfx)]
    \\
    +  \ctrlaff^\top \bfM_k(\bfx)^\top   K_{\grad \LieOne h}(\bfx, \bfx') \bfM_k(\bfx)\ctrlaff
\end{multline}

Recall that $\cov(\vect(\bfY), \vect(\bfX D)) =  \bfB_{\bfX, \bfY} D \otimes \bfA_{\bfX, \bfY}$, from  \eqref{eq:mean-var-grad-lie-grad-h-f-expanded}
\begin{multline}
    \cov(\grad \LieOne h(\bfx), \dynAff_k(\bfx) \ctrlaff) 
    \\
    = \calJ_\bfx[ \bfb_k(\bfx, \bfx') ]^\top \ctrlaff \otimes \grad_\bfx h(\bfx)^\top A
    \\
    + \bfb_k(\bfx, \bfx')^\top \ctrlaff \otimes \calH_{\bfx, \bfx} h(\bfx)^\top A.
\end{multline}
\begin{multline}
    \cov(\grad \LieOne h(\bfx), \dynAff_k(\bfx) \ctrlaff) 
    \\
    = \big(
    \calJ_\bfx[ \bfb_k(\bfx, \bfx') ]^\top \otimes \grad_\bfx h(\bfx)^\top A
    \\
    + \bfb_k(\bfx, \bfx')^\top \otimes \calH_{\bfx, \bfx} h(\bfx)^\top A 
    \big) \big( \ctrlaff \otimes I_{n \times n})
\end{multline}

Using the properties of trace $\tr(X+Y) = \tr(X) + \tr(Y)$ and that $\tr(\bfx \bfy^\top) = \bfy^\top \bfx$
\begin{multline}
    \tr(\cov(\grad \LieOne h(\bfx), \dynAff_k(\bfx) \ctrlaff) )
    \\
    = \grad_\bfx h(\bfx)^\top A \calJ_\bfx[ \bfb_k(\bfx, \bfx') ]^\top \ctrlaff 
    \\
    +  \tr(\calH_{\bfx, \bfx} h(\bfx)^\top A)\bfb_k(\bfx, \bfx')^\top \ctrlaff.
\end{multline}
\begin{multline}
    \tr(\cov(\grad \LieOne h(\bfx), \dynAff_k(\bfx) \ctrlaff) )^2
    \\
    = \ctrlaff^\top (\grad_\bfx h(\bfx)^\top A \calJ_\bfx[ \bfb_k(\bfx, \bfx') ]^\top)^2 \ctrlaff 
    \\
    +  \ctrlaff^\top \bfb_k(\bfx, \bfx')\tr(\calH_{\bfx, \bfx} h(\bfx)^\top A)^2\bfb_k(\bfx, \bfx')^\top \ctrlaff.
    \label{eq:var-lie2-trace-term}
\end{multline}

Focusing on the second term of \eqref{eq:lie-2-var-app},
\begin{multline}
    \E[\grad \LieOne h(\bfx)]^\top 
    \cov(\grad \LieOne h(\bfx), \dynAff_k(\bfx)\ctrlaff )
    \bfM_k(\bfx) \ctrlaff 
    \\
    = 
    \big( 
    \E[\grad \LieOne h(\bfx)]^\top  \calJ_\bfx[ \bfb_k(\bfx, \bfx') ]^\top \ctrlaff  \big) 
    \grad_\bfx h(\bfx)^\top A
    \bfM_k(\bfx) \ctrlaff 
    \\
    + \ctrlaff^\top \bfb_k(\bfx, \bfx')
    E[\grad \LieOne h(\bfx)]^\top  \calH_{\bfx, \bfx} h(\bfx)^\top A
    \bfM_k(\bfx) \ctrlaff 
    \\
    =
    \ctrlaff^\top \calJ_\bfx[ \bfb_k(\bfx, \bfx') ]\E[\grad \LieOne h(\bfx)]
    \grad_\bfx h(\bfx)^\top A
    \bfM_k(\bfx) \ctrlaff 
    \\
    + \ctrlaff^\top \bfb_k(\bfx, \bfx')
    E[\grad \LieOne h(\bfx)]^\top  \calH_{\bfx, \bfx} h(\bfx)^\top A
    \bfM_k(\bfx) \ctrlaff
    \label{eq:var-lie2-cov-term}
\end{multline}

Putting expanded terms from \eqref{eq:var-lie2-trace-term} and \eqref{eq:var-lie2-cov-term} into \eqref{eq:lie-2-var-app},
\begin{multline}
  \Var[\ctrlaff^\top \dynAff_k(\bfx)^\top \grad \LieOne  h(\bfx)]
  \\
  =
  % trace term
  2 \ctrlaff^\top (\grad_\bfx h(\bfx)^\top A \calJ_\bfx[ \bfb_k(\bfx, \bfx') ]^\top)^2 \ctrlaff 
  \\
    +  2 \ctrlaff^\top \bfb_k(\bfx, \bfx')\tr(\calH_{\bfx, \bfx} h(\bfx)^\top A)^2\bfb_k(\bfx, \bfx')^\top \ctrlaff
    \\
    % covariance term
    + 2  \ctrlaff^\top \calJ_\bfx[ \bfb_k(\bfx, \bfx') ]\E[\grad \LieOne h(\bfx)]
    \grad_\bfx h(\bfx)^\top A
    \bfM_k(\bfx) \ctrlaff 
    \\
    + 2 \ctrlaff^\top \bfb_k(\bfx, \bfx')
    E[\grad \LieOne h(\bfx)]^\top  \calH_{\bfx, \bfx} h(\bfx)^\top A
    \bfM_k(\bfx) \ctrlaff
    \\
    % Var(F(u)) term
    +  \ctrlaff^\top (\E[\grad \LieOne h(\bfx)]^\top \bfA \E[\grad \LieOne h(\bfx)]) \bfB  \ctrlaff
    \\
    % Var(F
    +  \ctrlaff^\top \bfM_k(\bfx)^\top   K_{\grad \LieOne h}(\bfx, \bfx') \bfM_k(\bfx)\ctrlaff
\end{multline}
\begin{multline}
  \ctrlaff^\top\Var[\dynAff_k(\bfx)^\top \grad \LieOne  h(\bfx)]\ctrlaff
  \\
    = \ctrlaff^\top \Big(
  2  (\grad_\bfx h(\bfx)^\top A \calJ_\bfx[ \bfb_k(\bfx, \bfx') ]^\top)^2  
  \\
    +  2  \bfb_k(\bfx, \bfx')\tr(\calH_{\bfx, \bfx} h(\bfx)^\top A)^2\bfb_k(\bfx, \bfx')^\top 
    \\
    % covariance term
    + 2   \calJ_\bfx[ \bfb_k(\bfx, \bfx') ]\E[\grad \LieOne h(\bfx)]
    \grad_\bfx h(\bfx)^\top A
    \bfM_k(\bfx)  
    \\
    + 2  \bfb_k(\bfx, \bfx')
    E[\grad \LieOne h(\bfx)]^\top  \calH_{\bfx, \bfx} h(\bfx)^\top A
    \bfM_k(\bfx) 
    \\
    +   (\E[\grad \LieOne h(\bfx)]^\top \bfA \E[\grad \LieOne h(\bfx)]) \bfB  
    \\
    +   \bfM_k(\bfx)^\top   K_{\grad \LieOne h}(\bfx, \bfx') \bfM_k(\bfx)
    \Big) \ctrlaff
  \label{eq:lie-2-var-app}
\end{multline}
    
\begin{multline}
  \cov(\LieOne h(\bfx), \grad \LieOne h(\bfx)^\top \dynAff(\bfx) \ctrlaff)
  \\
  =
    \cov(\LieOne h(\bfx), \grad \LieOne h(\bfx')) \bfM_0(\bfx)\ctrlaff
    \\
    + \cov(\LieOne h(\bfx), \dynAff(\bfx)\ctrlaff) \E[\grad \LieOne h(\bfx)]
\end{multline}
\begin{multline}
  =
    \cov(\LieOne h(\bfx), \grad \LieOne h(\bfx')) \bfM_0(\bfx)\ctrlaff
    \\
  + \grad h(\bfx)^\top \bfA (\bfb_k(\bfx, \bfx')^\top \ctrlaff)\E[\grad \LieOne h(\bfx)]
\end{multline}
\begin{multline}
  = 
    \cov(\LieOne h(\bfx), \grad \LieOne h(\bfx')) \bfM_0(\bfx)\ctrlaff
    \\
  + \grad h(\bfx)^\top \bfA \E[\grad \LieOne h(\bfx)] (\bfb_k(\bfx, \bfx')^\top \ctrlaff)
\end{multline}
\begin{multline}
  \cov( \grad \LieOne h(\bfx)^\top \dynAff(\bfx), \LieOne h(\bfx))
  \\
  =
    \bfM_0(\bfx)^\top \cov(\grad \LieOne h(\bfx'), \LieOne h(\bfx)) 
    \\
  + \grad h(\bfx)^\top \bfA \E[\grad \LieOne h(\bfx)] (\bfb_k(\bfx, \bfx'))
\end{multline}
\begin{multline}
  =
    \bfM_0(\bfx)^\top \Big( 
    \grad_\bfx b_{f_k}(\bfx, \bfx') \grad h(\bfx)^\top \bfA \grad h(\bfx') 
    \\
  + b_{f_k}(\bfx, \bfx') \grad h(\bfx') \bfA^\top \calH_{xx}[h(\bfx)]
    \Big)
    \\
  + \grad h(\bfx)^\top \bfA \E[\grad \LieOne h(\bfx)] (\bfb_k(\bfx, \bfx'))
  \label{eq:lie-2-lie-1-covar-app}
\end{multline}%
% 

==> tex/rem112.tex <==
\begin{remark}
\label{remar1!}
\rm{
Assuming  $\|\dot{x}(t_k)\|\neq0$ in Theorem~\eqref{ir5o45t!!!} is not restricting our results. Since, if the state of the system is safe and it does not change it remains safe. 

%As discussed, for consistent learning algorithm $p_k \rightarrow 1$ as $k \rightarrow \infty$. In this case as $T \rightarrow \infty$ for any $\epsilon >0$ there exist  $k_0 \in \mathbb{N}$ such that 
% \begin{align}
%     \prod_{k=k_0}^{\infty} p_k \ge 1-\epsilon.
% \end{align}
% In this case the controller $u$ renders the set $\mathcal{C}$ safe as time tends to infinity with probability at least 
%  \begin{align}
%     (1-\epsilon)\prod_{k=0}^{k_0} p_k.
% \end{align}
%
The lower bound~\eqref{lowerboun44!!22} is derived based on the independence of the events, it is not tight in general. In fact,
the chance constraint in program~\eqref{prog:CBF-CLF:unknown} can be replaced by
\begin{align}
   \mathbb{P}(\mbox{CBC}_k \ge \zeta | \bfx_k,\bfu_k, \mbox{CBC}_{k-1} \ge \zeta) \ge p_{k|k-1}, 
\end{align}
where $p_{k|k-1}$ is the lower bound of the chance constraint at $k$th triggering time provided that CBC was at least $\zeta$ in the $k-1$th triggering time, and $\mbox{CBC}_0$ is the value of CBC at time $0$. Assume the GP sample paths are sufficiently smooth such that there exist a sufficiently large $L_k$ for which the event~\eqref{eq:smoth23} occurs at all triggering time. Then the safety probability can be lower-bounded by  \begin{align}
 \prod_{k=1}^{N(T)} p_{k|k-1}.
 \end{align}
 As the controller observe more data, under BI, the posterior probability will concentrate on the true model. Thus, we can use tighter chance constraints in program~\eqref{prog:CBF-CLF:unknown}. 
 We leave these treatments for future research.
 }
 \end{remark}
